Fast and Correct Gradient-Based Optimisation for Probabilistic Programming via Smoothing

We study the foundations of variational inference, which frames posterior inference as an optimisation problem, for probabilistic programming. The dominant approach for optimisation in practice is stochastic gradient descent. In particular, a variant using the so-called reparameterisation gradient estimator exhibits fast convergence in a traditional statistics setting. Unfortunately, discontinuities, which are readily expressible in programming languages, can compromise the correctness of this approach. We consider a simple (higher-order, probabilistic) programming language with conditionals, and we endow our language with both a measurable and a smoothed (approximate) value semantics. We present type systems which establish technical pre-conditions. Thus we can prove stochastic gradient descent with the reparameterisation gradient estimator to be correct when applied to the smoothed problem. Besides, we can solve the original problem up to any error tolerance by choosing an accuracy coefficient suitably. Empirically we demonstrate that our approach has a similar convergence as a key competitor, but is simpler, faster, and attains orders of magnitude reduction in work-normalised variance.

==> backup/app-sau.tex <==
% !TEX root = ../main.tex

\subsection{Properties of Uniform Almost Uniform Convergence}

\dw{Sufficient if derivative of $\phi_\para$ has lower bound?}

\dw{$\rep_\para:\trsp\to\Real^n$, $\mu$ finite (or probability) measure on $\trsp$.}
\lo{What do we assume about $\rep_\para$? Strong diffeomorphism?}

Suppose $\mu(U)=\E_{\lat\sim\mdist}([\lat\in U])$, where $\mdist$ has finite moments.

\begin{lemma}
  \label{lem:balldim}
  $\lim_{k\in\nat}\sup_{\para\in\parasp}\mu(\rep_\para^{-1}(\Real^n\setminus\ball k))=0$
\end{lemma}

\begin{proof}
  Let $\lat_0\in\trsp$ be arbitrary.
  \renewcommand\ball[1]{\mathbf B_{#1}(\lat_0)}

  \begin{align*}
    \delta_*^{(i)}&\defeq\sup_{\para\in\parasp}|\rep_\para^{(i)}(\lat_0)|\\
    d_k^{(i)}&\defeq\sup_{\para\in\parasp}\sup_{\lat\in\ball k}\|\nabla_\para\rep^{(i)}_\para(\lat)\|
  \end{align*}
  thus if $\lat\in\ball k$,
  \begin{align*}
    |\rep_\para(\lat)^{(i)}|&\leq \|\rep^{(i)}_\para(0)\|+\langle\nabla\rep^{(i)}_\para(\zeta),x\rangle\\
    &\leq \delta_*^{i}+\|\nabla\rep^{(i)}_\para(\zeta)\|\cdot\|x\|\\
    &\leq \delta_*^{i}+ d_k^{(i)}\cdot k
  \end{align*}
  Let
  \begin{align*}
    \delta_k^{(i)}&\defeq \delta_*^{i}+ d_k^{(i)}\cdot k&
    \delta_k&\defeq\sqrt n\cdot\max_{i=1}^n\delta_k^{(i)}
  \end{align*}
  Note that for $\lat\in\Real^n$,
  if $\|\rep_\para(\lat)\|>\delta_k$ then $|\rep_\para^{(i)}(\lat)|>\delta_r^{(i)}$ for some $1\leq i\leq n$ and thus $\lat\in\Real^n\setminus\ball k$.
  As a consequence, $\rep_\para^{-1}(\Real^n\setminus\mathbf B_{\delta_k}(\mathbf 0))\subseteq\Real^n\setminus\ball k$.

  Now, it suffices to observe that $\lim_k\mu(\trsp\setminus\ball k)=0$. \dw{reason in opposite direction}
%  Now, it suffices to observe that $\nu_\para(\Real^n\setminus\ball k)\leq\int_{\Real^n\setminus \ball k}\nd(\lat)\cdot M\diff\lat$. \dw{general pdf}
\end{proof}

\iffalse
\begin{lemma}
  \label{lem:balldim}
  $U_k\defeq\trsp'\cap\ball k$
  Let $(U_k)_{k\in\nat}$ be a sequence of compact sets such that $\cup_{k\in\nat}U_k=\trsp'$.
Then
  $\lim_{k\in\nat}\sup_{\para\in\parasp}\mu(\rep_\para^{-1}(\trsp'\setminus U_k))$
\end{lemma}
\begin{proof}
  Let
  \begin{align*}
    \delta_*^{(i)}&\defeq\sup_{\para\in\parasp}|\rep_\para^{(i)}(\mathbf 0)|\\
    d_k^{(i)}&\defeq\sup_{(\para,\lat)\in\parasp\times U_k}\|\nabla_\para\rep^{(i)}_\para(\lat)\|
  \end{align*}
  thus if $\lat\in U_k$,
  \begin{align*}
    |\rep_\para(\lat)^{(i)}|&\leq \|\rep^{(i)}_\para(0)\|+\langle\nabla\rep^{(i)}_\para(\zeta),x\rangle\\
    &\leq \delta_*^{i}+\|\nabla\rep^{(i)}_\para(\zeta)\|\cdot\|x\|\\
    &\leq \delta_*^{i}+ d_k^{(i)}\cdot k
  \end{align*}
  Let
  \begin{align*}
    \delta_k^{(i)}&\defeq \delta_*^{i}+ d_k^{(i)}\cdot k&
    \delta_k&\defeq\sqrt n\cdot\max_{i=1}^n\delta_k^{(i)}
  \end{align*}
  Note that for $\lat\in\trsp$,
  if $\|\rep_\para(\lat)\|>\delta_k$ then $|\rep_\para^{(i)}(\lat)|>\delta_r^{(i)}$ for some $1\leq i\leq n$ and thus $\lat\in\trsp'\setminus U_k$.
  As a consequence, $\rep_\para^{-1}(\Real^n\setminus\ball{\delta_k})\subseteq\Real^n\setminus\ball k$.

  Now, it suffices to observe that $\lim_k\mu(\Real^n\setminus\ball k)=0$. \dw{reason in opposite direction}
%  Now, it suffices to observe that $\nu_\para(\Real^n\setminus\ball k)\leq\int_{\Real^n\setminus \ball k}\nd(\lat)\cdot M\diff\lat$. \dw{general pdf}
\end{proof}
\fi


\begin{lemma}
  For each $k\in\nat$ there exists $c>0$ such that $\mu(\rep^{-1}_\para(U\cap\ball k))\leq c\cdot\Leb(U\cap\ball k)$.
\end{lemma}
\begin{proof}
  Let $f:\Real^n\to\Real$ be the density of $\mu$ \dw{details}. Then
  \begin{align*}
    \mu(\rep^{-1}_\para(U\cap\ball k))&=\int_{\rep^{-1}_\para(U\cap\ball k)} f(\lat)\diff\lat\\
    &=\int_{U\cap\ball k} f(\rep^{-1}_\para(\repx))\cdot|\det\Jac\rep^{-1}_\para(\repx)|\diff\repx
  \end{align*}
  \dw{there exists upper bound by continuity of $\rep_\para^{-1}$}
\end{proof}

\begin{lemma}
  \label{lem:ausig}
  Suppose $f_\eta\circ\rep_{(-)}(-)\sau f\circ\rep_{(-)}(-)$ and $f\neq 0$ a.e.

  Then $\smooth\circ f_\eta\circ\rep_{(-)}(-)\sau [f(\rep_{(-)}(-))>0]$.
\end{lemma}
\begin{proof}
  Let $\delta_k$, $\epsilon_k$ and $\eta_k$ be witnesses for $f_\eta\circ\rep_{(-)}(-)\sau f\circ\rep_{(-)}(-)$.

  For $i\in\nat$ define $V_i\defeq\{\repx\in\Real^n\mid|f(\repx)|<\frac 1 i\}$.
  For every $k\in\nat$ there exists $i_k\in\nat$ such that $\Leb(V_{i_k}\cap\ball k)<\frac 1 k$.
    (This is because $\Leb((-)\cap\ball k)$ is a finite measure and $\cap_{i\in\nat} V_{i}\subseteq f^{-1}(0)$ and $f\neq 0$ a.e.)

  Furthermore, for $k\in\nat$ let $K_k\in\nat$ be such that $\epsilon_{K_k}<\frac 1{2{i_k}}$.
  By \cref{ass:sig} there exists $0<\eta_k'<\eta_{K_k}$ such that for all $0<\eta<\eta'_k$ and $y>\frac 1{2i_k}$, $\smooth(-y)<\frac 1 k$ and $\smooth(y)>1-\frac 1 k$.
  We also define
  \begin{align*}
    \delta'_k&\defeq\delta_{K_k}+\sup_{\para\in\parasp}\mu(\rep_\para^{-1}(\Real^n\setminus\ball k))+\frac 1 k&
    \epsilon'_k&\defeq\frac 1 k
  \end{align*}
  By \cref{lem:balldim}, $\lim\delta'_k=0=\lim\epsilon'_k$.

  Now, suppose $\para\in\parasp$ and $k\in\nat$.


  Define $U'\defeq U_{K_k}\cup\rep_\para^{-1}(V_{i_k})$ where $U_{K_k}\subseteq\Real^n$ is the corresponding set for $[f(\rep_{(-)}(-))>0]$, $\para$ and $K_k$.
  It holds
  \begin{align*}
    \mu(U')&\leq
    \mu(U_{K_k})+\mu(\rep_\para^{-1}(\Real^n\setminus\ball{k}))+\mu(\rep_\para^{-1}(V_{i_k}\cap\ball{k}))\\
    &\leq\mu(U_{K_k})+\mu(\rep_\para^{-1}(\Real^n\setminus\ball{k}))+c\cdot\Leb(V_{i_k}\cap\ball{k})\\
    &\leq\delta'_k
  \end{align*}
  \dw{$c$, make sure it works}
  Besides,
  for $0<\eta<\eta_k'$ and $\lat\in\Real^n\setminus U'$,
  $|f_\eta(\rep_\para(\lat))-f(\rep_\para(\lat))|<\frac 1{2i_k}$ and $|f(\rep_\para(\lat))|\geq\frac 1{i_k}$ thus
  $|f_\eta(\rep_\para(\lat))|>\frac 1{2{i_k}}$.

  Consequently, $|\smooth(f_\eta(\rep_\para(\lat)))-[f(\rep_\para(\lat))>0]|<\frac 1 k$.
\end{proof}


\begin{lemma}
  \label{lem:aucomp}
  If $f:U_1\times U_2\to\Real$ (for open and \changed[dw]{connected} $U_1,U_2\subseteq\Real$) is continuously differentiable and $g_\eta\sau g:\Real^n\to U_1$ and $h_\eta\sau h:\Real^n\to U_2$, \changed[dw]{$g,h$ are also bounded on bounded subsets of $\Real^n$} then $f\circ\langle g_\eta,h_\eta\rangle\sau f\circ\langle g,h\rangle:\Real^n\to\Real$ \changed[dw]{is also bounded on bounded subsets of $\Real^n$}.
\end{lemma}
\begin{proof}
  First, note that $f\circ\langle g,h\rangle$ is bounded on bounded subsets of $\Real^n$ because $f$ is continuously differentiable and $g$ and $h$ also satisfies this property.

  Let $\delta_k^{(i)}$, $\epsilon_k^{(i)}$ and $\eta_k^{(i)}$ ($i\in\{1,2\}$) be witnesses for $g_\eta\sau g$ and $h_\eta\sau h$.
  W.l.o.g.\ all $\epsilon_k^{(i)}\leq 1$.
  Observe that for $k\in\nat$,
  \begin{align*}
    M_k&\defeq \sup_{(\para,\lat)\in\parasp\times\ball k} \|(g(\para,\lat),h(\para,\lat))\|+\sqrt 2<\infty
  \end{align*}
  because
  $g(\parasp\times\ball k)$ and $h(\parasp\times\ball k)$ are bounded by assumption (also \cref{ass:comp}).
  and therefore
  \begin{align*}
    d_k&\defeq\sup_{(x,y)\in M_k\cap(U_1\times U_2)}\left\|\nabla f(x,y)\right\|<\infty
  \end{align*}
   is well-defined.
  For $k\in\nat$ there exists $K_k\geq k$ such that each
  $\sqrt 2\cdot d_k\cdot\epsilon_{K_k}^{(i)}<\frac 1 k$.

  Define
  \begin{align*}
    \delta_k&\defeq\mu(\Real^n\setminus\ball k)+\delta^{(1)}_{K_k}+\delta^{(2)}_{K_k}&
    \epsilon_k&\defeq\frac 1 k&
    \eta_k&\defeq\min\{\eta_{K_k}^{(1)},\eta_{K_k}^{(2)}\}
  \end{align*}
  Note that by \cref{lem:balldim}, $\lim\delta_k=0=\lim\epsilon_k$.

  Let $\para\in\parasp$ and $k\in\nat$.
  Let $V\defeq (\Real^n\setminus\ball k)\cup V^{(1)}\cup V^{(2)}$, where $V^{(1)}$ (and $V^{(2)}$, respectively) are the sets for $g$ (and $h$, respectively), $\para$ and $K_k$.
  Note that $\mu(V)\leq\delta_k$. Besides for every $0<\eta<\eta_k$ and $\lat\in\Real^n\setminus V$,
  $|g_\eta(\para,\lat)|\leq|g(\para,\lat)|+\epsilon_{K_k}^{(1)}\leq|g(\para,\lat)|+1$ (similarly for $h$). Hence,
  every point between $(g_\eta(\para,\lat),h_\eta(\para,\lat))$ and $(g(\para,\lat),h(\para,\lat))$ is in $\ball {M_k}\cap(U_1\times U_2)$ and therefore by the mean value theorem,
  \begin{align*}
    &\left|f(g_\eta(\para,\lat),h_\eta(\para,\lat))-f(g(\para,\lat),h(\para,\lat))\right|\\
    &\leq
    \sup_{\zeta\in \ball {M_k}\cap(U_1\times U_2)}\left|\left\langle\nabla f(\zeta),\left(g_\eta(\para,\lat)-g(\para,\lat),h_\eta(\para,\lat)-h(\para,\lat)\right)\right\rangle\right|\\
    &\leq\sup_{\zeta\in \ball {M_k}\cap(U_1\times U_2)}\|\nabla f(\zeta)\|\cdot
    \left\|\left(g_\eta(\para,\lat)-g(\para,\lat),h_\eta(\para,\lat)-h(\para,\lat)\right)\right\|&\text{Cauchy–Schwarz inequality}\\
    &< d_k\cdot\sqrt{2}\cdot\max\{\epsilon_{K_k}^{(1)},\epsilon_{K_k}^{(2)}\}\\
    &\leq\epsilon_k
    &&%\qedhere READD
%     \sum_{i=1}^\ell d^{(i)}\left|g_\eta^{(i)}(\para,\lat)-g^{(i)}(\para,\lat)\right|\leq\epsilon_k
  \end{align*}
\end{proof}

% \dw{easier to just prove for primitives?}
% \begin{corollary}
%   \label{cor:sauop}
%   For $+,\cdot,-,{}^{-1},\exp,\log$.
% \end{corollary}

\iffalse
\begin{lemma}
  \label{lem:aucomp}
  If $f:\Real_{e_1}\times\cdots\times\Real_{e_\ell}\to\Real$ is continuously differentiable and $g_\eta^{(1)}\sau g^{(1)}:\trsp\to\Real_{e_1},\ldots,g_\eta^{(\ell)}\sau g^{(\ell)}:\trsp\to\Real_{e_\ell}$ \dw{$g^{(i)}$ also bounded on bounded subsets of $\trsp$} then $f\circ\langle g_\eta^{(1)},\ldots,g_\eta^{(\ell)}\rangle\sau f\circ\langle g^{(1)},\ldots,g^{(\ell)}\rangle:\trsp\to\Real$ \dw{also bounded on bounded subsets of $\trsp$}.
\end{lemma}
\begin{proof}
  First, note that $f\circ\langle g^{(1)},\ldots,g^{(\ell)}\rangle$ is bounded on bounded subsets of $\trsp$ because $f$ is continuously differentiable and $g^{(i)}$ also satisfies this property.

  Let $\delta_k^{(i)}$, $\epsilon_k^{(i)}$ and $\eta_k^{(i)}$ be for $g^{(i)}$.

  Let
  \begin{align*}
    d_k\defeq\sup_{(\para,\lat)\in\parasp\times\ball k}\left\|\nabla f(g^{(1)}(\para,\lat),\ldots,g^{(\ell)}(\para,\lat))\right\|<\infty
  \end{align*}
  \dw{gradient of $f$}
  which is well-defined because for each $k\in\nat$,  each $g^{(j)}(\parasp\times\ball k)$ is bounded by assumption. \dw{$\parasp$ is compact}
  For $k\in\nat$ there exists $K_k\geq k$ such that each
  $d_k\cdot\epsilon_{K_k}^{(i)}<\frac 1 k$.

  Define
  \begin{align*}
    \delta_k&\defeq\mu(\trsp\setminus\ball k)+\sum_{i=1}^\ell \delta^{(i)}_{K_k}\\
    \epsilon_k&\defeq\frac 1 k\\
    \eta_k&\defeq\min_{i=1}^\ell\eta_{K_k}^{(i)}\\
  \end{align*}
  Note that $\lim\delta_k=0=\lim\epsilon_k$.

  Let $\para\in\parasp$ and $k\in\nat$.
  Let $U\defeq (\trsp\setminus\ball k)\cup U^{(1)}\cup\cdots\cup U^{(\ell)}$, where $U^{(j)}$ are the sets for $g^{(i)}$ and $K_k$.
  Note that $\mu(U)\leq\delta_k$. Besides for every $0<\eta<\eta_k$ and $\lat\in\trsp\setminus U$,
  \begin{align*}
    &\left|f(g_\eta^{(1)}(\para,\lat),\ldots,g_\eta^{(\ell)}(\para,\lat))-f(g^{(1)}(\para,\lat),\ldots,g^{(\ell)}(\para,\lat))\right|\\
    &\leq
    \left\langle\nabla f(g^{(1)}(\para,\lat),\ldots,g^{(\ell)}(\para,\lat)),\left(g_\eta^{(1)}(\para,\lat)-g^{(1)}(\para,\lat),\ldots,g_\eta^{(\ell)}(\para,\lat)-g^{(\ell)}(\para,\lat)\right)\right\rangle\\
    &\leq\|\nabla f(g^{(1)}(\para,\lat),\ldots,g^{(\ell)}(\para,\lat))\|\cdot
    \left\|\left(g_\eta^{(1)}(\para,\lat)-g^{(1)}(\para,\lat),\ldots,g_\eta^{(\ell)}(\para,\lat)-g^{(\ell)}(\para,\lat)\right)\right\|\\
    &\leq d_k\cdot\max_{i=1}^k\epsilon_{K_k}^{(i)}\\
    &\leq\epsilon_k
%     \sum_{i=1}^\ell d^{(i)}\left|g_\eta^{(i)}(\para,\lat)-g^{(i)}(\para,\lat)\right|\leq\epsilon_k
  \end{align*}
\end{proof}

\begin{lemma}
  \label{lem:aucl}
  \dw{subsumed by \cref{lem:aucomp}}
  If $f_\eta\sau f$ and $g_\eta\sau g$ then $f_\eta+g_\eta\sau f+g$ and $f_\eta\cdot g_\eta\sau f\cdot g$.
\end{lemma}
\begin{proof}
  Addition should be easy.

  For multiplication, let $\epsilon_k^{(1)},\epsilon_k^{(2)}$ and $\delta_k^{(1)},\delta_k^{(2)}$ and $\eta_k^{(1)},\eta_k^{(2)}$ be the sequences for $f$ and $g$, respectively. \dw{W.l.o.g.\ decreasing}

    W.l.o.g.\ $\epsilon_k^{(2)}<1$ for all $k\in\nat$.

    Let $M_k>0$ be such that $\mu(\Real^n\setminus\ball{M_k})<\frac 1 k$.
  Define
  \begin{align*}
    c_k\defeq\max\left\{\sup_{(\para,\lat)\in\parasp\times\ball{M_k}}|f(\para,\lat)|,\sup_{(\para,\lat)\in\parasp\times\ball{M_k}}|g(\para,\lat)|+1\right\}
  \end{align*}
  (which is well-defined because $f$ and $g$ are \changed[dw]{bounded by polynomials} and \changed{$\ball{M_k}$ is bounded}.)

  There exists $K_k\geq k$ such that $\epsilon_{K_k}^{(1)},\epsilon_{K_k}^{(2)}<\frac 1{k\cdot c_k}$.

  We define
  \begin{align*}
    \delta_k&\defeq\delta_{K_k}^{(1)}+\delta_{K_k}^{(2)}+\frac 1 k\\
    \epsilon_k&\defeq\frac 2 k\\
    \eta_k&\defeq\min\{\eta_k^{(1)},\eta_k^{(2)}\}
  \end{align*}
  Clearly, $\lim\delta_k=0=\lim\epsilon_k$.

  Now, let $k\in\nat$ and $\para\in\parasp$. Let $U_{K_k}^{(1)}$ and $U_{K_k}^{(2)}$ be for $K_k$, $f$ and $g$.
  That is:
  \begin{enumerate}
    \item $\Leb(U_{K_k}^{(1)})<\delta^{(1)}_{K_k}$ and $\Leb(U_{K_k}^{(2)})<\delta^{(2)}_{K_k}$
    \item $|f_\eta(\para,\lat)-f(\para,\lat)|<\epsilon_{K_k}^{(1)}$ for every $0<\eta<\eta_{K_k}^{(1)}$ and $\lat\in \Real^n\setminus U_{K_k}^{(1)}$
    \item $|g_\eta(\para,\lat)-g(\para,\lat)|<\epsilon_{K_k}^{(2)}$ for every $0<\eta<\eta_{K_k}^{(2)}$ and $\lat\in \Real^n\setminus U_{K_k}^{(2)}$
  \end{enumerate}
  In particular, $|g_\eta(\para,\lat)|<|g(\para,\lat)|+\epsilon_{K_k}^{(2)}<c_k$ for every $0<\eta<\eta_{K_k}^{(2)}$ and $\lat\in\ball{M_k}\setminus U_{K_k}^{(2)}$.


  Define $U\defeq (\Real^n\setminus\ball{M_k})\cup U_{K_k}^{(1)}\cup U_{K_k}^{(2)}$. Note that $\mu(U)<\delta_k$.
  Besides, for $0<\eta<\eta_k$ and $\lat\in\Real^n\setminus U_k$,
  \begin{align*}
    &|f_\eta(\para,\lat)\cdot g_\eta(\para,\lat)-f(\para,\lat)\cdot g(\para,\lat)|\\
    &\leq
    |f_\eta(\para,\lat)-f(\para,\lat)|\cdot|g_\eta(\para,\lat)|+
    |f(\para,\lat)|\cdot|g_\eta(\para,\lat)-g(\para,\lat)|\\
    &\leq \epsilon_{K_k}^{(1)}\cdot c_k+c_k\cdot\epsilon_{K_k}^{(2)}\\
    &\leq\epsilon_k
  \end{align*}
\end{proof}



\subsection{Uniform Convergence of Gradient}
\begin{proposition}
  $\para\mapsto\E_{\lat\sim\mdist}\left[\frac{\partial\sema\SFC}{\partial\theta_i}(\para,\lat)\right]$ converges uniformly on $\parasp$.
\end{proposition}
\begin{proof}
  \begin{enumerate}
    \item Consider $\ifc\SFC\SFCb\SFCc$.
    \begin{align*}
      &\E_{\lat\sim\mdist}\left[\frac{\partial\sema{\ifc\SFC\SFCb\SFCc}}{\partial\theta_i}(\para,\lat)\right]\\
      &=\E_{\lat\sim\mdist}\left[\frac{\partial(\smooth\circ(-\sema\SFC)}{\partial\theta_i}(\para,\lat)\cdot\sema\SFCb(\para,\lat)\right]+
      \E_{\lat\sim\mdist}\left[\frac{\partial(\smooth\circ\sema\SFC)}{\partial\theta_i}(\para,\lat)\cdot\sema\SFCc(\para,\lat)\right]\\
      &+\E_{\lat\sim\mdist}\left[\smooth(-\sema\SFC(\para,\lat))\cdot\frac{\partial\sema\SFCb}{\partial\theta_i}(\para,\lat)\right]
      +\E_{\lat\sim\mdist}\left[\smooth(\sema\SFC(\para,\lat))\cdot\frac{\partial\sema\SFCc}{\partial\theta_i}(\para,\lat)\right]
    \end{align*}
    The uniform convergence of the latter two terms follows easily \dw{reference}.
    For the others note there exists $\psi_\eta:\Real^n\to\Real$ \dw{type} and $\rep_\para$ such that
    $\sema\SFC=\psi_\eta\circ\rep_\para$. \dw{reference lemmas}
    \begin{align*}
      &\E_{\lat\sim\mdist}\left[\frac{\partial(\smooth\circ\sema\SFC)}{\partial\theta_i}(\para,\lat)\cdot\sema\SFCc(\para,\lat)\right]\\
      &=\E_{\lat\sim\mdist}\left[\frac{\partial(\smooth\circ\psi_\eta\circ\rep_\para)}{\partial\theta_i}(\para,\lat)\cdot\sema\SFCc(\para,\lat)\right]\\
      &=\sum_{j=1}^n\E_{\lat\sim\mdist}\left[\chi_{i,j}(\para,\lat)\cdot\frac{\partial(\smooth\circ\psi_\eta\circ\rep_\para)}{\partial z_j}(\para,\lat)\cdot\sema\SFCc(\para,\lat)\right]\\
      &=\sum_{j=1}^n\E_{\lat_{-j}\sim\mdist_{-j}}\left[\underbrace{\left[\pdf_{\dist_j}(z_j)\cdot\chi_{i,j}(\para,\lat)\cdot\smooth(\psi_\eta(\rep_\para(\para,\lat)))\cdot\sema\SFCc(\para,\lat)\right]_{-\infty}^\infty}_0\right]\\
      &+\sum_{j=1}^n\E_{\lat_{-j}\sim\mdist_{-j}}\left[\int\smooth(\psi_\eta(\rep_\para(\para,\lat)))\cdot\frac{\partial}{\partial z_j}\left(\sema\SFCc(\para,\lat)\cdot\pdf_{\dist_j}(z_j)\cdot\chi_{i,j}(\para,\lat)\right)\diff z_j\right]
    \end{align*}
    \dw{need log}
    \dw{justify}
  \end{enumerate}
\end{proof}

\subsection{Bounded Variance}

\newcommand\good[1]{\xrightarrow{#1}}
\dw{notation}
\changed[dw]{$f_\eta\good\ell f:\parasp\times\trsp\to\Real$ if $f_\eta\sau f$, $\E_\lat[|\log^\ell(f(\para,\lat))|]<\infty$, $\E_\lat[\nabla\|\log^\ell(f(\para,\lat))\|]<\infty$.
}

Suppose $f,g:\Real^2\to\Real_{>0}$. Note that
\begin{align*}
  \left|\frac{\partial(\log \circ (f+g))}{\partial x}(x,y)\right|&=\left|\frac{\frac{\partial (f+g)}{\partial x}(x,y)}{f(x,y)+g(x,y)}\right|\\
  &\leq\left|\frac{\frac{\partial f}{\partial x}(x,y)}{f(x,y)+g(x,y)}\right|+\left|\frac{\frac{\partial g}{\partial x}(x,y)}{f(x,y)+g(x,y)}\right|\\
  &\leq\left|\frac{\frac{\partial f}{\partial x}(x,y)}{f(x,y)}\right|+\left|\frac{\frac{\partial g}{\partial x}(x,y)}{g(x,y)}\right|\\
  &\leq\left|\frac{\partial(\log \circ f)}{\partial x}(x,y)\right|+\left|\frac{\partial(\log \circ g)}{\partial x}(x,y)\right|
\end{align*}
Besides, inductively, for all $\ell\in\nat$ and $f,g:\Real^2\to\Real_\ell$,
\begin{align}
  \label{eq:logder}
  \left|\frac{\partial(\log^\ell \circ (f+g))}{\partial x}(x,y)\right|\leq\left|\frac{\partial(\log^\ell \circ f)}{\partial x}(x,y)\right|+\left|\frac{\partial(\log^\ell \circ g)}{\partial x}(x,y)\right|
\end{align}
\begin{align*}
  \left|\frac{\partial(\log^{\ell+1} \circ (f+g))}{\partial x}(x,y)\right|=
  \left|\frac {\frac{\partial(\log^\ell \circ (f+g))}{\partial x}(x,y)}{\log^\ell(f(x,y)+g(x,y))}\right|\\
  &\leq\left|\frac {\frac{\partial(\log^\ell \circ f)}{\partial x}(x,y)}{\log^\ell(f(x,y)+g(x,y))}\right|+
  \left|\frac {\frac{\partial(\log^\ell \circ g)}{\partial x}(x,y)}{\log^\ell(f(x,y)+g(x,y))}\right|\\
  &\leq\left|\frac {\frac{\partial(\log^\ell \circ f)}{\partial x}(x,y)}{\log^\ell(f(x,y))}\right|+
  \left|\frac {\frac{\partial(\log^\ell \circ g)}{\partial x}(x,y)}{\log^\ell(g(x,y))}\right|\\
  &=\left|\frac{\partial(\log^{\ell+1} \circ f)}{\partial x}(x,y)\right|+\left|\frac{\partial(\log^{\ell+1} \circ g)}{\partial x}(x,y)\right|
\end{align*}
\begin{lemma}
  Let $\para,\lat\mid[]\vdash\SFC:\bt\PCFReal e\Delta$. Then $\E[|\frac {\partial(\log^\ell\circ\sema\SFC)}{\partial\theta_i}(\para,\lat)|]<\infty$. \dw{uniform}
\end{lemma}
\begin{proof}
  \begin{enumerate}
    \item Suppose $\para,\lat\mid[]\vdash\SFC+\SFCb:\bt e\ell\Delta$ because $\para,\lat\mid[]\vdash\SFC:\bt e\ell\Delta$ and $\para,\lat\mid[]\vdash\SFCb:\bt e\ell\Delta$. It holds
    \begin{align*}
      \E[|\frac {\partial(\log^\ell\circ\sema{\SFC+\SFCb})}{\partial\theta_i}(\para,\lat)|]&\leq
      \E[|\frac {\partial(\log^\ell\circ\sema\SFC)}{\partial\theta_i}(\para,\lat)|+|\frac {\partial(\log^\ell\circ\sema\SFCb)}{\partial\theta_i}(\para,\lat)|]\\
      &\leq\E[|\frac {\partial(\log^\ell\circ\sema{\SFC})}{\partial\theta_i}(\para,\lat)|]+
      \E[|\frac {\partial(\log^\ell\circ\sema{\SFCb})}{\partial\theta_i}(\para,\lat)|]
      <\infty
    \end{align*}
    by \cref{eq:logder} and assumption.
    \item For $\ifc\SFC\SFCb\SFCc$. \changed[dw]{We focus on the case $\ell=1$ for now.}
    \begin{align*}
      &\E\left[\left|\frac{\partial(\log\circ\sema{\ifc\SFC\SFCb\SFCc})}{\partial\theta_i}(\para,\lat)\right|\right]\\
      &=\E\left[\left|\frac{\frac{\partial(\smooth\circ(-\sema\SFC))}{\partial\theta_i}(\para,\lat)\cdot\sema\SFCb(\para,\lat)+\frac{\partial(\smooth\circ\sema\SFC)}{\partial\theta_i}(\para,\lat)\cdot\sema\SFCc(\para,\lat)+\smooth(-\sema\SFC(\para,\lat))\cdot\frac{\partial\sema\SFCb}{\partial\theta_i}(\para,\lat)+\smooth(\sema\SFC(\para,\lat))\cdot\frac{\partial\sema\SFCc}{\partial\theta_i}(\para,\lat)}{\sema{\ifc\SFC\SFCb\SFCc}(\para,\lat)}\right|\right]\\
      &\leq\E\left[\left|\frac{\frac{\partial(\smooth\circ(-\sema\SFC))}{\partial\theta_i}(\para,\lat)\cdot\sema\SFCb(\para,\lat)+\frac{\partial(\smooth\circ\sema\SFC)}{\partial\theta_i}(\para,\lat)\cdot\sema\SFCc(\para,\lat)}{\sema{\ifc\SFC\SFCb\SFCc}(\para,\lat)}\right|\right]\\
      &+\E\left[\left|\underbrace{\frac{\smooth(-\sema\SFC(\para,\lat))\cdot\frac{\partial\sema\SFCb}{\partial\theta_i}(\para,\lat)}{\smooth(-\sema\SFC(\para,\lat))\cdot\sema\SFCb(\para,\lat)}}_{\frac{\partial(\log\cdot\sema\SFCb)}{\partial\theta_i}(\para,\lat)}\right|\right]+\E\left[\left|\underbrace{\frac{\smooth(\sema\SFC(\para,\lat))\cdot\frac{\partial\sema\SFCc}{\partial\theta_i}(\para,\lat)}{\smooth(\sema\SFC(\para,\lat))\cdot\sema\SFCc(\para,\lat)}}_{\frac{\partial(\log\cdot\sema\SFCc)}{\partial\theta_i}(\para,\lat)}\right|\right]\\
      &\leq 2c+\E\left[\left|\frac{\nabla_\lat(\smooth\circ(-\sema\SFC))(\para,\lat)\cdot\vel_i(\para,\lat)\cdot\sema\SFCb(\para,\lat)+\nabla_\lat(\smooth\circ\sema\SFC)(\para,\lat)\cdot\vel_i(\para,\lat)\cdot\sema\SFCc(\para,\lat)}{\sema{\ifc\SFC\SFCb\SFCc}(\para,\lat)}\right|\right]\\
      &\leq 2c+\sum_{j=1}^n\E\left[\left|\chi_{i,j}(\para,\lat)\cdot\frac{\frac{\partial(\smooth\circ(-\sema\SFC))}{\partial z_j}(\para,\lat)\cdot\sema\SFCb(\para,\lat)+\frac{\partial(\smooth\circ\sema\SFC)}{\partial z_j}(\para,\lat)\cdot\sema\SFCc(\para,\lat)}{\sema{\ifc\SFC\SFCb\SFCc}(\para,\lat)}\right|\right]\\
      &\leq 2c+\sum_{j=1}^n\E\left[\left|\chi_{i,j}(\para,\lat)\cdot\frac{\partial(\log\circ\sema{\ifc\SFC\SFCb\SFCc})}{\partial z_j}(\para,\lat)\right|\right]\\
      &+\sum_{j=1}^n\E\left[\left|\chi_{i,j}(\para,\lat)\cdot\underbrace{\frac{\smooth(-\sema\SFC(\para,\lat))\cdot\frac{\partial\sema\SFCb}{\partial z_j}(\para,\lat)}{\sema{\ifc\SFC\SFCb\SFCc}(\para,\lat)}}_{\leq\left|\frac{\partial(\log\circ\sema\SFCb)}{\partial z_j}(\para,\lat)\right|}\right|\right]+\sum_{j=1}^n\E\left[\left|\chi_{i,j}(\para,\lat)\cdot\underbrace{\frac{\smooth(\sema\SFC(\para,\lat))\cdot\frac{\partial\sema\SFCc}{\partial z_j}(\para,\lat)}{\sema{\ifc\SFC\SFCb\SFCc}(\para,\lat)}}_{\leq\left|\frac{\partial(\log\circ\sema\SFCc)}{\partial z_j}(\para,\lat)\right|}\right|\right]
    \end{align*}
    which is sufficient because $\E[|\chi_{i,j}(\para,\lat)|]<c$.
  \end{enumerate}
\end{proof}

\fi


==> backup/app-type.tex <==
% !TEX root = ../main.tex

\begin{lemma}
  \label{cor:form}
  If the properties in \cref{prop:form} hold then
  \begin{enumerate}
    \item $\log^e\circ\sem M$ is bounded by a polynomial \dw{where needed, find good statemtent}
    \item for each $\eta>0$, partial derivatives of $\log^e\circ\sema M$ up to order $2$ are bounded by a polynomial uniformly in $\para\in\parasp$
    \item $\log^e\circ\sema M\sau\log^e\circ\sem M$ \dw{need to omit log?}
    \item if $g=1$ then $\log^e\circ\sem M= f\circ\rep_{(-)}$, $\log^e\circ\sema M= f_\eta\circ\rep_{(-)}$ and $f\neq 0$ a.e.\ and $\boundary f^{-1}[0,\infty)$ is negligible \lo{What is $f$?} \dw{measure} \dw{justify} \dw{and state properties}
  \end{enumerate}
\end{lemma}
\dw{justify}
\dw{why boundary negligible if $\PCFRp$?}


==> backup/experiments.tex <==
% !TEX root = ../main.tex

\dw{constant vs.\ decreasing step size}

%\lo{TODO: Below lifted from IMCL22 submission / Basim's disseertation. TODO: produce plots with \textsc{Product} estimator removed.}

We evaluate our smoothed gradient estimator and Diagonalisation Stochastic Gradient Descent  (\textsc{Smooth}) against the biased reparameterisation estimator (\textsc{Reparam}), the unbiased correction of it (\textsc{Lyy18}) due to \cite{LYY18}, and the unbiased (\textsc{Score}) estimator \cite{RGB14,WW13,DBLP:conf/icml/MnihG14}.
The implementation is written in Python, using automatic differentiation (provided by the \texttt{jax} library) to implement each of the above estimators for an arbitrary probabilistic program.

\dw{DISCUSS: variance vs.~approximation error}


\changed[dw]{
\paragraph{Compilation for First-Order Programs}
\label{sec:comp}

All our benchmarks are first-order. We can compile a potentially discontinuous program to a smooth program (parametrised by $\smooth$) using the compatible closure of
\begin{align*}
  \ifc LMN\rightsquigarrow (\lambda w\ldotp \smooth(-w)\cdot M+\smooth(w)\cdot N)\,L
\end{align*}
Note that the size only increases linearly and that we avoid of an exponential blow-up by using abstractions rather than duplicating the guard $L$.
}
\iffalse
\begin{proposition}
  If $M\rightsquigarrow N$ then $\sema M=\sema N$. For every $M$ there exists a normal form $N$ w.r.t.\ $\rightsquigarrow$ and $\sema M=\sem N$. \dw{doesn't make sense because in different categories}
\end{proposition}
As a consequence, we can compile the program to its smoothing and use standard automatic differentiation libraries.
\dw{perhaps describe in implementation section?}
\lo{Possibly. One argument for it is that the low-order nature of development is acceptable (and arguably natural) in the context of empirical validation (the crucial examples from LYY18 are all first order).}
\fi



\subsection{Models}

\newcommand\lyy{\hbox{\textsc{Lyy18} }}
\renewcommand\score{\hbox{\textsc{Score} }}
\newcommand\nested{\hbox{\textsc{Smooth} }}
\newcommand\reparam{\hbox{\textsc{Reparam }}}

We include the models from \cite{LYY18}, which are as follows:

\begin{itemize}
  \item \texttt{temperature} \cite{DBLP:conf/qest/SoudjaniMN17} models a controller keeping the temperature of a room within set bounds.
  The discontinuity arises from the discrete state of the controller, being either on or off, which disrupts the continuous state representing the temperature of the room.
  Given a set of noisy measurements of the room temperature, the goal is to infer the controller state at each of 21 time steps. The model has a 41-dimensional latent variable and 80 if-statements.

  \item \texttt{textmsg} \cite{DavidsonPilon15} models daily text message rates, and the goal is to discover a change in the rate over the 74-day period of data given.
  The non-differentiability arises from the point at which the rate is modelled
  to change. The model has a 3-dimensional latent variable (the two rates and
  the point at which they change) and 37 if-statements.

  \item \texttt{influenza}  \cite{ShumwayS05} models the US influenza mortality for
  1969.
  In each month, the mortality rate depends on the dominant virus strain being of type 1 or type 2, producing a non-differentiablity for each month.
  Given the mortality data, the goal is to infer the dominant virus strain in each month. The model has a 37-dimensional latent variable and 24 if-statements.
\end{itemize}

Additionally, we introduce the following models:

\begin{itemize}
  \item \texttt{cheating} %, adapted from the book \emph{Bayesian Methods for Hackers}
  \cite{DavidsonPilon15} simulates a differential privacy setting where students taking an exam are surveyed to determine the prevalence of cheating without exposing the details for any individual.
  Students are tasked to toss a coin, on heads they tell the truth (cheating or not cheating) and on tails they toss a second coin to determine their answer.
  The tossing of coins here is a source of discontinuity.
  The goal, given the proportion of students who answered yes, is to predict a posterior on the cheating rate.
  In this model there are 300 if-statements and a 301-dimensional latent space, although we only optimise over a single dimension with the other 300 being sources of randomness.

  \item \texttt{xornet} is a simple multi-layer neural network trained to compute the exclusive-or (XOR) function.
  It has a \changed[lo]{\texttt{2-4-2-1}} network architecture with two inputs and one output, and all activation functions being the Heaviside step function which is traditionally infeasible for gradient-based optimisation because of the discontinuity at $0$ and a zero gradient everywhere else.
  The model has a \changed[lo]{25-dimensional} latent space (for all the weights and biases) and 28 if-statements.
  Note that this model is not applicable to the \lyy estimator since the branch conditions are not all affine in the latent space.
\end{itemize}

\subsection{Experimental Setup}
\label{sec:expt-setup}

The experimental setup was based on that of \cite{LYY18}.
For each estimator and model, we used the Adam \cite{DBLP:journals/corr/KingmaB14} optimiser for $10,000$ iterations using a learning rate of $0.001$, with the exception of \texttt{xornet} for which we used $0.01$.
The initial model parameters $\para_0$ were fixed for each model across all runs.
In each iteration, we used $N \in \{1,8,16\}$ Monte Carlo samples from the gradient estimator.
For the \lyy estimator, a single subsample for the boundary term was used in each estimate.
For our smoothed estimator and Diagonalisation Stochastic Gradient Descent, we use the smoothing trajectory: $\eta_k = \frac{10}{\sqrt k}$, here $10$ was chosen to work well across all models.
%For the \product estimator, we used a single subsample for the Monte Carlo approximation and all experiments in this section were done using the control variate mentioned in Section \cref{sec:product-smooth}.

To generate the ELBO trajectories shown in \cref{fig:estimator variance}, we separately took 1000 samples of the ELBO every 100 iterations, taking extra samples to reduce the variance in the graphs presented.
The random samples were the same across estimators, which leads to the correlation in noise seen in their trajectories.

\cref{tab:var} compares the average variance of the estimators, where the average is taken over a single optimisation trajectory.
For each estimator, we took 1000 Monte Carlo samples of the gradient every 100 iterations to compute the variance of the estimator at that iteration; we then computed the average of these variances.
Since the gradients are vectors, the variance was measured in two ways: averaging the component-wise variances and the variance of the $L_2$ norm.

We then separately benchmark each estimator by measuring how many iterations each can complete in a fixed time budget and setting the computational cost to be the reciprocal of that.
This is then used to compute a \emph{work-normalised variance} \cite{glynn1992asymptotic,Botev2017} that is taken to be the product of the computational cost and variance.
Intuitively, we divide by the relative time taken since we can reduce the variance by the same factor running the faster estimator more times.

\subsection{Analysis of Results}

%Our \texttt{jax} implementation of the \textsc{Lyy18} estimator followed the inventors' implementation as closely as possible, so we believe it is a fair comparison point.

The ELBO graph for the \texttt{temperature} model in \cref{fig:temperature-graph} shows that the \reparam estimator is biased, converging to a suboptimal value when compared to the \nested and \lyy estimators.
We can also see from the graph and the data in \cref{tab:temperature} that the \score estimator exhibits extremely high variance, and does not converge.
%Between the smoothed estimators, \product converges faster although \nested exhibits a lower variance. One possible hypothesis for this could be that the particular form of smoothing done by \nested gives more of a gap between the smoothed gradient and the true gradient.
%\lo{Include variance data for \score in \cref{tab:var} (which can be up to $10^{-10}$ times larger)?}

The \texttt{textmsg} and \texttt{influenza} ELBO graphs in \cref{fig:textmsg-graph} and \cref{fig:influenza-graph} both show all estimators converging towards roughly the same value, with \score exhibiting a larger variance.
The work-normalised variance of the \nested estimator across both model is the lowest across both variance measures.

For the \texttt{cheating} model in \cref{fig:cheating-graph}, we have another visual indicator of the bias of the \reparam gradient.
%Here the high number of conditionals (300 if-statements) in the model likely contribute to the high variance exhibited by Monte Carlo approximation in the \product estimator, resulting in similar trajectory to \score but a worse work-normalised variance in \cref{tab:cheating} when we take into account the extra computational cost.
Here \nested outperforms again with the lowest work-normalised variance (ignoring that of \reparam since it is biased).

Finally, the \texttt{xornet} model shows the difficulty of training step-function based neural nets.
The \lyy estimator is not applicable here since the boundary integral has no general efficient estimator for non-affine conditionals, which is the case here.
In \cref{fig:xornet-graph}, the \reparam estimator makes no progress while other estimators manage to converge to close to $0$ ELBO, showing that they learn a network that correctly classifies all points.
In particular, the \nested estimator converges the quickest.

To summarise, the results show cases where the \reparam estimator is biased and how the \nested estimator do not have the same limitation.
Where the \lyy estimator is defined, they converge to roughly the same objective value; and the smoothing approach is generalisable to more complex models such as neural networks with non-linear boundaries.
Our proposed \nested estimator has consistently significantly lower work-normalised variance, up to 3 orders of magnitude.

%% Format testing

\begin{figure}[ht]
  \centering
  %\small
  \begin{subfigure}[h]{.48\textwidth}
    \includegraphics[width=\linewidth]{figures/output_4_1.png}
    \caption{\texttt{temperature}}
    \label{fig:temperature-graph}
  \end{subfigure}
\quad
  \begin{subfigure}[h]{.48\textwidth}
    \includegraphics[width=\linewidth]{figures/output_5_1.png}
    \caption{\texttt{textmsg}}
    \label{fig:textmsg-graph}
  \end{subfigure}
\\
\vspace*{10pt}
\begin{subfigure}[h]{.48\textwidth}
  \includegraphics[width=\linewidth]{figures/output_6_1.png}
  \caption{\texttt{influenza}}
  \label{fig:influenza-graph}
\end{subfigure}
\quad
\begin{subfigure}[h]{.48\textwidth}
  \includegraphics[width=\linewidth]{figures/output_7_1.png}
  \caption{\texttt{cheating}}
  \label{fig:cheating-graph}
\end{subfigure}
\\
\vspace*{10pt}
\begin{subfigure}[h]{.48\textwidth}
  \includegraphics[width=\linewidth]{figures/output_8_1.png}
  \caption{\texttt{xornet}}
  \label{fig:xornet-graph}
\end{subfigure}
\caption{ELBO trajectories for each model. A single colour is used for each
  estimator and the accuracy coefficient $\eta=0.1,0.15,0.2$ for \textsc{Smooth} is represented by dashed, solid and
  dotted lines respectively. \label{fig:estimator variance}}
\end{figure}


%%% FORMATTING TESTING

\begin{table}[ht]
  \caption{Computational cost and work-normalised variances, all given as ratios
  with respect to the \textsc{Score} estimator (whose data are omitted since they would be a row of $1$s).}
  \label{tab:var}
  \centering
 \small
%  \vspace*{5pt}
  \begin{subtable}[h]{.4\textwidth}
    \caption{\texttt{temperature}}
    \label{tab:temperature}
    \centering
    \begin{tabular}{lcccr}
      \toprule
      Estimator & Cost & $\textrm{Avg}(V(.))$ & $V(\|.\|_2)$ \\
      \midrule
      \textsc{Smooth} & 3.27e+00 & 2.90e-10 & 2.18e-09 \\
      %\textsc{Product} & 1.31e+01 & 1.08e-06 & 2.33e-05 \\
      \textsc{Reparam} & 1.51e+00 & 1.40e-08 & 1.96e-08 \\
      \textsc{Lyy18} & 1.06e+01 & 2.78e-07 & 9.43e-06 \\
      \bottomrule
    \end{tabular}
  \end{subtable}
\qquad\qquad
%  \vspace*{10pt}
  \begin{subtable}[h]{.4\textwidth}
    \caption{\texttt{textmsg}}
    \label{tab:textmsg}
    \centering
    \begin{tabular}{lcccr}
      \toprule
      Estimator & Cost & $\textrm{Avg}(V(.))$ & $V(\|.\|_2)$ \\
      \midrule
      \textsc{Smooth} & 2.07e+00 & 4.70e-02 & 4.82e-02 \\
      %\textsc{Product} & 3.00e+00 & 4.26e-01 & 4.65e-01 \\
      \textsc{Reparam} & 1.36e+00 & 3.69e-02 & 3.66e-02 \\
      \textsc{Lyy18} & 2.50e+00 & 7.95e-02 & 7.24e-02 \\
      \bottomrule
    \end{tabular}
  \end{subtable}
\\
 \vspace*{10pt}
  \begin{subtable}[h]{.4\textwidth}
    \caption{\texttt{influenza}}
    \label{tab:influenza}
    \centering
    \begin{tabular}{lcccr}
      \toprule
      Estimator & Cost & $\textrm{Avg}(V(.))$ & $V(\|.\|_2)$ \\
      \midrule
      \textsc{Smooth} & 1.73e+00 & 7.59e-03 & 3.78e-03 \\
      %\textsc{Product} & 4.22e+00 & 1.59e-01 & 1.61e-01 \\
      \textsc{Reparam} & 1.45e+00 & 6.62e-03 & 3.22e-03 \\
      \textsc{Lyy18} & 1.02e+01 & 5.32e-02 & 2.61e-02 \\
      \bottomrule
    \end{tabular}
  \end{subtable}
\qquad\qquad
%  \vspace*{10pt}
  \begin{subtable}[h]{.4\textwidth}
    \caption{\texttt{cheating}}
    \label{tab:cheating}
    \centering
    \begin{tabular}{lcccr}
      \toprule
      Estimator & Cost & $\textrm{Avg}(V(.))$ & $V(\|.\|_2)$ \\
      \midrule
      \textsc{Smooth} & 1.67e+00 & 5.47e-03 & 8.44e-03 \\
      %\textsc{Product} & 2.12e+00 & 4.28e+00 & 8.30e+00 \\
      \textsc{Reparam} & 6.63e-01 & 1.70e-19 & 4.10e-19 \\
      \textsc{Lyy18} & 2.03e+00 & 1.11e-01 & 2.50e-01 \\
      \bottomrule
    \end{tabular}
  \end{subtable}
\\
\vspace*{10pt}
  \begin{subtable}[h]{.5\textwidth}
    \caption{\texttt{xornet}}
    \label{tab:xornet}
    \centering
    \begin{tabular}{lcccr}
      \toprule
      Estimator & Cost & $\textrm{Avg}(V(.))$ & $V(\|.\|_2)$ \\
      \midrule
      \textsc{Smooth} & 1.89e+00 & 8.09e-03 & 8.59e-02 \\
      %\textsc{Product} & 2.21e+00 & 1.56e-01 & 1.28e+00 \\
      \textsc{Reparam} & 3.03e-01 & 1.93e-09 & 9.72e-10 \\
      \bottomrule
    \end{tabular}
  \end{subtable}
\end{table}
%%%

\iffalse
%% lifted from Basim's dissertation
\begin{table}[ht]
  \caption{Computational cost and work-normalised variances, all given as ratios
  with respect to the \textsc{Score} estimator (omitted since it would be all
  $1$s).}
  \label{tab:var}

  \large

  \vspace*{5pt}
  \begin{subtable}{\linewidth}
    \caption{\texttt{temperature}}
    \label{tab:temperature}
    \centering
    \begin{tabular}{lcccr}
      \toprule
      Estimator & Cost & $\textrm{Avg}(V(.))$ & $V(\|.\|_2)$ \\
      \midrule
      \textsc{Smooth} & 3.27e+00 & 2.90e-10 & 2.18e-09 \\
      %\textsc{Product} & 1.31e+01 & 1.08e-06 & 2.33e-05 \\
      \textsc{Reparam} & 1.51e+00 & 1.40e-08 & 1.96e-08 \\
      \textsc{Lyy18} & 1.06e+01 & 2.78e-07 & 9.43e-06 \\
      \bottomrule
    \end{tabular}
  \end{subtable}

  \vspace*{10pt}
  \begin{subtable}{\linewidth}
    \caption{\texttt{textmsg}}
    \label{tab:textmsg}
    \centering
    \begin{tabular}{lcccr}
      \toprule
      Estimator & Cost & $\textrm{Avg}(V(.))$ & $V(\|.\|_2)$ \\
      \midrule
      \textsc{Smooth} & 2.07e+00 & 4.70e-02 & 4.82e-02 \\
      %\textsc{Product} & 3.00e+00 & 4.26e-01 & 4.65e-01 \\
      \textsc{Reparam} & 1.36e+00 & 3.69e-02 & 3.66e-02 \\
      \textsc{Lyy18} & 2.50e+00 & 7.95e-02 & 7.24e-02 \\
      \bottomrule
    \end{tabular}
  \end{subtable}

  \vspace*{10pt}
  \begin{subtable}{\linewidth}
    \caption{\texttt{influenza}}
    \label{tab:influenza}
    \centering
    \begin{tabular}{lcccr}
      \toprule
      Estimator & Cost & $\textrm{Avg}(V(.))$ & $V(\|.\|_2)$ \\
      \midrule
      \textsc{Smooth} & 1.73e+00 & 7.59e-03 & 3.78e-03 \\
      %\textsc{Product} & 4.22e+00 & 1.59e-01 & 1.61e-01 \\
      \textsc{Reparam} & 1.45e+00 & 6.62e-03 & 3.22e-03 \\
      \textsc{Lyy18} & 1.02e+01 & 5.32e-02 & 2.61e-02 \\
      \bottomrule
    \end{tabular}
  \end{subtable}

  \vspace*{10pt}
  \begin{subtable}{\linewidth}
    \caption{\texttt{cheating}}
    \label{tab:cheating}
    \centering
    \begin{tabular}{lcccr}
      \toprule
      Estimator & Cost & $\textrm{Avg}(V(.))$ & $V(\|.\|_2)$ \\
      \midrule
      \textsc{Smooth} & 1.67e+00 & 5.47e-03 & 8.44e-03 \\
      %\textsc{Product} & 2.12e+00 & 4.28e+00 & 8.30e+00 \\
      \textsc{Reparam} & 6.63e-01 & 1.70e-19 & 4.10e-19 \\
      \textsc{Lyy18} & 2.03e+00 & 1.11e-01 & 2.50e-01 \\
      \bottomrule
    \end{tabular}
  \end{subtable}

  \vspace*{10pt}
  \begin{subtable}{\linewidth}
    \caption{\texttt{xornet}}
    \label{tab:xornet}
    \centering
    \begin{tabular}{lcccr}
      \toprule
      Estimator & Cost & $\textrm{Avg}(V(.))$ & $V(\|.\|_2)$ \\
      \midrule
      \textsc{Smooth} & 1.89e+00 & 8.09e-03 & 8.59e-02 \\
      %\textsc{Product} & 2.21e+00 & 1.56e-01 & 1.28e+00 \\
      \textsc{Reparam} & 3.03e-01 & 1.93e-09 & 9.72e-10 \\
      \bottomrule
    \end{tabular}
  \end{subtable}
\end{table}

\fi

%Finally, our \texttt{jax} implementation of the \textsc{Lyy18} estimator followed the inventors' implementation as closely as possible so we claim it is a fair comparison point.
%To support our claim, in the supplementary material we include results from adding our \textsc{Smooth} estimator to the code made publicly available by \citet{LYY18} and show that the results are still comparable. \lo{TODO: Add this to the Appendix.}


==> backup/intro.tex <==
% !TEX root = ../main.tex

In probabilistic programming and Bayesian machine learning we are often interested in minimising (or maximising) expectations of the form
\begin{align}
  \label{eq:info}
  \text{argmin}_\para\,\E_{\lat\sim q{(\lat)}}[f(\para,\lat)]
\end{align}
%i.e.\ we seek parameters $\para^\ast$ minimising (or maximising) that expectation.
We are especially interested in scenarios in which the function $f$ is directly expressed in a programming language.
(Our ultimate goal is to target languages for constructing applications in numerical analysis and computational science such as Julia \cite{Julia-2017} %\footnote{\url{https://julialang.org/}}
or in Bayesian statistics and probabilistic programming such as Stan~\cite{stan} and Pyro~\cite{pyro}.)
Owing to the presence of conditionals, the function $f$ may not be continuous, let alone differentiable.
Also note that the distribution $q(\lat)$ (with respect to which the expectation is taken) is independent of the parameters $\para$.

\subsection*{Variational Inference, ELBO and Reparameterisation Gradient Estimator}

The archetypical example of objective function of the form in \cref{eq:info} is the \emph{Evidence Lower Bound} (ELBO)\footnote{This is so for the ELBO \emph{after reparameterisation}, for example \cref{eq:reparam example from sd}; notice that the distribution in \cref{eq:ELBO} still depends on the parameters $\para$.}, which plays a pivotal role in variational inference \cite{Zhang2019,Murphy2012,B07}.
In the variational inference approach to Bayesian statistics, the problem of approximating difficult-to-compute posterior probability distributions is transformed to an optimisation problem.
The idea is to approximate the posterior probability $p(\repx \mid \mathbf x)$ using a family of ``simpler'' densities $q_\para(\repx)$ over the latent variables $\repx$, parameterised by $\para$.
The optimisation problem is then to find the parameter $\para^\ast$ that maximises the ELBO function
\begin{equation}
\mathrm{ELBO}_\para :=
\E_{\repx\sim q_\para{(\repx)}}[f(\para, \repx)]
\hbox{  where  }
f(\para, \repx) = \log p(\mathbf x,\repx)-\log q_\para(\repx)
\label{eq:ELBO}
\end{equation}
which is equivalent to the problem of finding the parameter $\para^\ast$ whereby the variational approximant $q_{\para^\ast}(\repx)$ is closest to the posterior distribution $p(\repx \mid \mathbf x)$ in KL-divergence \cite{Murphy2012,B07}.

To solve the optimisation problem, we want an efficient method to estimate the gradient of $\hbox{ELBO}_\para$.
The \emph{reparameterisation gradient estimator}---the dominant approach in variational inference---reparameterises the latent variable $\repx$ in terms of a base random variable $\lat$ (viewed as the entropy source) via a diffeomorphic transformation $\phi_\para$, such as a location-scale transformation or cumulative distribution function.
For example, if the distribution of the latent variable $\alpha$ is a Gaussian $\mathcal{N}(\alpha \mid \mu, \sigma^2)$ with parameters $\para = \{\mu,\sigma^2\}$ then the location-scale transformation using the standard normal as the base distribution gives rise to the reparameterisation
\[
\alpha \sim \mathcal{N}(\alpha \mid \mu, \sigma^2)
\iff
\alpha = \mu + \sigma \, {z}, \quad z \sim \nd(0,1).
\]
%\dw{Is the red for submission, or a workaround for a deficiency of the commenting package?} \lo{The latter. Now removed.}
% \lo{Good changes above - thanks!
% I also had it in mind to change the latent variable to another variable ($\not=$ $\lat$), so that it is clear that we use $z$ for the entropy source (which is to be reparameterised), $z \sim \nd(0,1)$, throughout.
% I think I remarked earlier that it was a bit confusing before.}
The key advantage of this setup (often called ``reparameterisation trick'' \cite{DBLP:journals/corr/KingmaW13,DBLP:conf/icml/TitsiasL14,DBLP:conf/icml/RezendeMW14}) is that we can now differentiate (by backpropagation) with respect to the parameters $\para$ of the variational distributions using Monte Carlo simulation with draws from the base distribution $\lat$.
Thus, succinctly, where $f(\theta, \alpha)$ is (the so-called \emph{instantaneous ELBO}) as defined in \cref{eq:ELBO}, we have
% \changed[dw]{
\begin{align}
\nabla_\para \,\hbox{ELBO}_\para
=
\nabla_\para\, \E_{\alpha \sim q_\para{(\alpha)}}[f(\para,\alpha)]
& =
\nabla_\para\, \E_{z \sim \nd(0, 1)}[f(\para,\mu + \sigma \, z)] \nonumber \\
& =
\E_{z \sim \nd(0,1)}[\nabla_\para f(\para, \mu + \sigma \, z)]
\label{eq:reparam example from sd}
\end{align}
The last equality, which commutes differentiation and integration, is a consequence of the dominated convergence theorem \cite[Theorem 6.28]{K13}.
\changed[lo]{Notice that the distribution of the expectation in \cref{eq:reparam example from sd} is independent of the parameter $\para$.}
% }
% \dw{@LO: What do you think about this change of notation? This is how it's currently used in the rest of the paper.}
% \lo{This is definitely clearer. See my preceding comment.}
% \lo{In posterior inference, both KL-divergence and ELBO have the form $\E_{\lat\sim q_\para(\lat)}[f(\para,\lat)]$ where $f$ is $\log q_\para(\lat)-\log p(\lat \mid \mathbf x)$ for the former, and $\log p(\lat, \mathbf x) - \log q_\para(\lat)$ for the latter (see \href{https://www.cs.ox.ac.uk/teaching/materials20-21/SPP/Lectures/7-Variational.pdf}{Slide 21/38}).
% The key advantage of ELBO is the use of joint (as opposed to conditional) density.
% Using KL-divergence as our example could be confusing / attract criticisms.}
% \dw{Yes, you are of course right. I've changed it back.}

Whilst it is less widely applicable than the SCORE estimator \cite{RGB14,WW13,DBLP:conf/icml/MnihG14}, the main benefit of the reparameterisation gradient estimator is that it has a significantly lower variance, resulting in faster convergence.
% \dw{reference}\lo{They would be the same references for the reparameterisation trick / gradient estimator. I think it unnecessary to repeat them here, as this is a well-known fact.}

\dw{Even the \textsc{SCORE} estimator may be biased for discontinuous \emph{guides} despite the myth that it is always applicable (cf.~\cite{LYRY19}).}

\subsection*{Gradient Based Optimisation}
Unfortunately, since $\E_{\lat\sim q(\lat)}[f(\para,\lat)]$ may not be a convex function, we cannot hope to always find global optima.
We seek instead \emph{stationary points}, where the gradient w.r.t.~the parameters $\para$ vanishes.

In practice, variants of \defn{Stochastic Gradient Descent (SGD)} are frequently employed, which converge to critical points under certain conditions \cite{RM51}. In its simplest form, SGD follows Monte Carlo estimates of the gradient in each step:
\begin{align*}
  \para_{k+1}&\defeq\para_k-\gamma_k\cdot\underbrace{\frac 1 N\sum_{i=1}^N\nabla_\theta f\left(\para_k,\lat_k^{(i)}\right)}_{\text{reparameterisation gradient estimator}}
\end{align*}
where $\lat_k^{(i)}\sim q\left(\lat_k^{(i)}\right)$ and $\gamma_k$ is the step size.


\iffalse
\lo{MINOR: Small clash of $\alpha_k$ with newly introduced latent variable $\alpha$, but ok as we don't use $\alpha$ anymore?}
\dw{You're right, thanks for spotting this, I would propose to use $\gamma$ for the step size.}
\fi
% Since, $f$ is expressed in a programming language it is typically not differentiable, let alone continuous.
% It is well-known that the reparameterisation gradient estimator \cite{LYY18,KW13,DBLP:conf/icml/TitsiasL14,RMW14} is biased for non-differentiable models \cite{LYY18}.
% Unfortunately, this may compromise convergence to critical points or minimisers.

In particular, a condition for convergence to critical points is unbiasedness of the gradient estimator \ref{it:sgdunb}.
% Due to the presence of conditionals in programming languages, $f$ is typically not continuous, let alone differentiable.\lo{repetition}
Unfortunately, the reparameterisation gradient estimator
% \cite{LYY18,KW13,DBLP:conf/icml/TitsiasL14,RMW14}
is biased for non-differentiable models \cite{LYY18}, which are readily expressible in programming languages with conditionals:
\begin{example}
  \label{ex:biased}
  The counterexample in \cite[Proposition~2]{LYY18}, where the objective function is the ELBO for a non-differentiable model, can be simplified to
  \begin{align*}
    f(\theta,z)&= -0.5\cdot\theta^2+
    \begin{cases}
      0&\tif z+\theta<0\\
      1&\tow
    \end{cases}
  \end{align*}
  Observe that (see \cref{fig:biased}):
  \[
    \nabla_\theta\,\E_{z\sim\nd(0,1)}\left[f(\theta,z)\right]
    =
    -\theta+\nd(-\theta\mid 0,1)
    \neq
    -\theta
    =
    \E_{z\sim\nd(0,1)}\left[\nabla_\theta f(\theta,z)\right]
  \]
  \iffalse
    \begin{align*}
      \nabla_\theta\,\E_{z\sim\nd(0,1)}\left[f(\theta,z)\right]&=-\theta+\nd(-\theta\mid 0,1)\\
      &\neq -\theta=
      \E_{z\sim\nd(0,1)}\left[\nabla_\theta f(\theta,z)\right]
    \end{align*}
  \fi
\end{example}
  % (\cref{ex} captures the essence of their counterexample.)
Unfortunately \emph{this may compromise convergence to critical points or maximisers}:
even if we can find a point where the gradient estimator vanishes, it may not be a critical point of the \emph{original} problem \eqref{eq:info}.

% Vanishing gradient estimator does \emph{not imply stationarity}!

\begin{figure}
  \centering
  \begin{tikzpicture}
    \begin{axis}[
      height=5cm,
      axis lines = middle,
      xlabel = \(\theta\),
      %      ylabel = {\(f(x)\)},
      ]
      %Below the red parabola is defined
      \addplot [
      domain=-1:1,
      samples=100,
      color=oxred,
      dashed,
      thick
      ]
      {-x};
      %    \addlegendentry{\(-\theta\)}
      %Here the blue parabola is defined
      \addplot [
      update limits=false,
      domain=-1:1,
      samples=100,
      color=oxgreen,
      thick
      ]
      {-x+1/sqrt(2*pi)*exp(-0.5*x*x)};
      %      \addlegendentry{\(-\theta+\nd(-\theta\mid 0,1)\)}
    \end{axis}
  \end{tikzpicture}
  \caption{Dashed red: biased estimator $\E_{z\sim\nd(0,1)}\left[\nabla_\theta f(\theta,z)\right]$, solid green: true gradient $\nabla_\theta\,\E_{z\sim\nd(0,1)}\left[f(\theta,z)\right]$ for \cref{ex:biased}.}
  \label{fig:biased}
\end{figure}


\subsection*{Our Approach}

\begin{figure}
  \hfill
  \begin{center}
    \begin{subfigure}[t]{0.4\linewidth}
      \begin{center}
        \begin{tikzpicture}
          \begin{axis}[
            ymin=-0.1,
            ymax=1.1,
            height=4.5cm,
            axis lines = middle,
            ]
            \addplot [
            domain=-1:0,
            samples=100,
            color=oxred,
            line width=0.3mm
            ]
            {{0}};
            \addplot [
            domain=0:1,
            samples=100,
            color=oxred,
            line width=0.3mm
            ]
            {{1}};

            \addplot [
            domain=-1:1,
            samples=100,
            line width=0.3mm,
            dotted
            ]
            {{1/(1+exp(-3*x))}};

            \addplot [
            update limits=false,
            domain=-1:1,
            samples=100,
            line width=0.3mm,
            dashed
            ]
            {1/(1+exp(-15*x))};
          \end{axis}
        \end{tikzpicture}
      \end{center}

      \caption{$\smooth$ (black, dashed/dotted) and the Heaviside step function (red, solid)}
      \label{fig:sigf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.4\linewidth}
      \begin{center}
        \begin{tikzpicture}
          \begin{axis}[
            ymin=-0.1,
            ymax=3.95,
            height=4.5cm,
            axis lines = middle,
            ]

            \addplot [
            domain=-1:1,
            samples=100,
            line width=0.3mm,
            dotted
            ]
            {{3/(1+exp(-3*x))*1/(1+exp(3*x))}};

            \addplot [
            update limits=false,
            domain=-1:1,
            samples=100,
            line width=0.3mm,
            dashed
            ]
            {15/(1+exp(-15*x))*1/(1+exp(15*x))};
          \end{axis}
        \end{tikzpicture}
      \end{center}
      \caption{Derivatives of $\sigma_k$}
      \label{fig:sigd}
    \end{subfigure}
    \hfill
    \caption{(Logistic) sigmoid function $\smooth$ and its derivative (dotted: $\eta=\frac 1 3$, dashed: $\eta=\frac 1{15}$).}
    \label{fig:sig}
  \end{center}
\end{figure}
\dw{reference \cref{fig:sig}}

% \dw{also needs to be updated}
Our method is based on an efficiently computable smoothed semantics of programs.
In particular, for \emph{accuracy coefficient} $\eta>0$, we interpret conditionals $M\equiv\ifc{z+\theta}{\underline 0}{\underline 1}$ as
\begin{gather*}
  \sema M(\theta,z)\defeq\smooth(z+\theta)
\end{gather*}
where $\smooth$ is a smooth function. For instance we can choose $\smooth(z)\defeq\sigma(\frac z\eta)$ where $\sigma(x) \defeq \frac 1{1+\exp(-x)}$ is the (logistic) sigmoid function.
Thus, the program $M$ is interpreted by a smooth function $\sema M$, for which the reparameterisation gradient can be estimated unbiasedly. Furthermore, employing a refinement type system, we establish that \emph{typabable} terms not only yield well-defined optimisation problems (as the expectation in \cref{eq:info} may be infinite) but that stochastic gradient descent converges to stationary points of the \emph{smoothed} problem.

Finally, we prove that the gradients for the smoothed problem converge \emph{uniformly} (in the parameters) to the gradient of the original optimisation problem \cref{eq:info}, which potentially involves discontinuities.
This provides a theoretical foundation for finding stationary points in \cref{eq:info}:
\begin{quote}
Given any error tolerance $\epsilon>0$ there is an accuracy coefficient $\eta>0$ such that a stationary point $\para^*$  of the $\eta$-smoothed problem have a gradient-norm of at most $\epsilon$ for the discontinuous problem \cref{eq:info}.
\end{quote}
Crucially, we can use \emph{convergent} stochastic gradient descent with the \emph{unbiased} reparametrisation gradient estimator for the $\eta$-smoothed problem.

  % , for which convergence results are well-established.
  % Therefore, we propose to apply a stochastic gradient descent-like procedure which enhances the accuracy coefficient $k$ in each step.

% \begin{enumerate}
%   \item \emph{Smoothen} (discontinuous) function using sigmoid with accuracy coefficient
%   \item Optimise expectation, enhancing accuracy in each step
% \end{enumerate}

\dw{plot \cref{fig:biased} for different accuracy coefficients}

% \dw{discuss polynomials, restriction on guards}

\iffalse
\lo{Hopefully Basim can exhibit empirically that running (DSGD') on the term \Cref{eq:counter eg} converges to the stationary point of the original optimisation problem, which is around $0.3722$, as $\nd(- 0.3722\mid 0,1) \approx 0.3722$.

Question: What happens when we run (SGD) on the LYY18 estimator of this term? Does it converge to the correct stationary point?
The point is that no proof exists that running (SGD) on the LYY18 estimator necessarily converges to a stationary point.
Do you think we might find a counterexample to the convergence of LYY18 estimator under (SGD)?

Reviewers of our paper will naturally compare our main contribution (provable convergence of (DDGS') to stationary points of an unbiased gradient estimator for typable programs) with the unbiased LYY18 estimator. The plus side: guaranteed convergence. Any negatives? Variance (work normalised) is still unknown.}
\fi

\subsection*{Contributions}
Our main contribution is the development and correctness proof of a novel \emph{end-to-end} optimisation method for expectations of the form \cref{eq:info} in the context of \emph{discontinuous} functions.
%This problem prominently arises in variational inference for probabilistic programming.
\changed[lo]{This addresses a major problem in variational inference for probabilistic programming.}

We employ a type system to guarantee that the optimisation problem for typabable programs can be solved \emph{up to any error tolerance} using an \emph{unbiased} reparametrisation gradient estimator, which exhibits good variance, for a \emph{smoothed} problem and stochastic gradient descent, which is guaranteed to \emph{converge}.


% We replace the discontinuous problem with a smooth problem, for which stochastic gradient works \dw{continue}

% unbiased variant, a problem arising in variational inference for probabilistic programs. extend the reparametrisation to discontinuous models using smooth approximations whilst enjoying unbiasedness.

% \emph{provable} convergence of a novel variant of SGD, \emph{Diagonalisation Stochastic Gradient Descent}, to stationary points for models defined by typable programs. The method takes gradient steps of a \emph{smoothed} model whilst simulatiously enhancing the accuracy of the approximation in each iteration.

% \dw{accuracy coefficient}

To formalise the approach, we present a simple (higher-order) programming language with conditionals.
We employ \emph{trace types} to capture precisely the samples drawn in a fully eager call-by-value evaluation strategy.

We endow our language with both a (measurable) denotational value semantics and a smoothed (hence approximate) value semantics.
In particular, for \emph{accuracy coefficient} $\eta>0$, we interpret conditionals using smooth functions.
For example
\begin{gather*}
  \sema {\ifc{z+\theta}{\underline 0}{\underline 1}}(\theta,z)\defeq \smooth(z+\theta)
\end{gather*}
%where $\smooth(z)\defeq\sigma(\frac z\eta)=\frac 1{1+\exp(-\frac z\eta)}$.
% where $\smooth(x)\defeq\sigma(\sqrt k\cdot x)=\frac 1{1+\exp(-\sqrt k\cdot x)}$ .

We also present a refinement type system which enforces mild restrictions on guards of conditionals and the magnitude of the expressible functions. This guarantees desirable properties in the context of our optimisation framework for typable programs:
\begin{enumerate}
  \item the objective function is well defined
  \item for each accuracy coefficient we obtain unbiased gradient estimators and show convergence of stochastic gradient descent
  \item the smoothed gradients converge uniformly to the true gradient as the accuracy is improved.
\end{enumerate}
thus providing the theoretical foundation for solving problems as in \cref{eq:info} for discontinuous problems readily expressible in programming languages.

% For the smoothed problems we obtain unbiased gradient estimators, which converge uniformly to the true gradient as the accuracy is improved.
%\lo{More explanation needed here.}

Finally we present empirical results showing that our unbiased estimator exhibits a similar convergence to the unbiased correction of the reparameterised gradient estimator by \cite{LYY18} -- our main baseline.
However our estimator is simpler and more efficient: it is faster and attains orders of magnitude (2 to 3,000 x) reduction in work-normalised variance. \dw{check}

\iffalse
\lo{
\begin{itemize}
  \item To formalise the problem, we consider a simple (higher-order, probabilistic) programming language with conditionals, and a type system enforcing a mild restriction on the parameters and a boundedness condition on the program's density function. \lo{Say what are the allowed primitive functions}

  \item We endow our language with a \emph{smoothed} (value) semantics parameterised by an accuracy coefficient.

  \item We present a novel variant of SGD, \emph{Diagonalisation Stochastic Gradient Descent} (DSGD), which sharpens the accuracy whilst taking gradient steps, and we prove convergence to stationary points for models definable by typable programs. \lo{Distinctives of the proof: use of Schwartz functions and tempered distributions}

  \item For the smoothed problems we obtain unbiased gradient estimators (for Problem \ref{eq:info}), which converge uniformly to the true gradient as the accuracy coefficient is raised.

  \item Our experiments show that our smoothed estimator enjoys a similarly low variance as the reparameterisation gradient estimator, whilst remaining unbiased for non-differentiable models.

  \item Compared to the unbiased correction of the reparameterised gradient estimator \cite{LYY18}, our estimator has a similar convergence, but is simpler, faster, and attains orders of magnitude (2 to 3,000 x) reduction in work-normalised variance.
\end{itemize}
}
\fi
\dw{Informal description, what happens if fixed smoothing is used.}

\paragraph{Outline}
In \cref{sec:prelims} we discuss some technical preliminaries. In \cref{sec:PL} we introduce a simple higher-order probabilistic programming language, its denotational value semantics and operational semantics; Optimisation \cref{p:opt} is then stated.
Also presented is a smoothed denotational value semantics, and we state the Smooth Optimisation \cref{p:optsm}.
In \cref{sec:types} we introduce a refinement type system that constraints the programming language.
In \cref{sec:type soundness,sec:prop} we show type soundness: refinement typable terms have a simple canonical form and satisfy the basic properties required for a SGD-like solution of the Optimisation Problem.
In \cref{sec:DSGD} we introduce the novel Diagonalisation Stochastic Gradient Descent algorithm.
In \cref{sec:empirical}, we present the results of our empirical evaluation, comparing the performance of our smoothed estimator with a number of baselines.
Related work is briefly discussed in \cref{sec:related}.
Finally, in \cref{sec:conclusion}, we conclude and discuss future directions.


==> backup/prelims.tex <==
% !TEX root = ../main.tex
\label{sec:prelims}

% \subsection{Stochastic Gradient Descent}
%
% \dw{state convergence and assumptions}

\iffalse
\subsection{Schwartz Functions}

We review some fundamental properties of Schwartz functions (see also for more details e.g.\ \cite{H15,R03} or \cite[App.~A]{G11}), abstract notions from functional analysis which turn out to be useful to organise our proofs.

\subsubsection{Schwartz Functions}

A smooth function $f:\Real^n\to\Real$ is a \defn{Schwartz function} if for all $\alpha$ and $\beta$ (using standard multi-index notation for higher-order partial derivatives),
\begin{align*}
  \sup_{\mathbf x\in\Real^n}|\mathbf x^\beta\cdot D^\alpha f(\mathbf x)|<\infty
\end{align*}
We use $\Schwsp(\Real^n)$ for the space of such Schwartz functions.
Intuitively, a Schwartz function decreases rapidly.

In this work we are particularly interested in Schwartz functions which are also the probability density function (pdf) \dw{w.r.t.\ Leb} of a continuous probability distribution. We call such functions \defn{Schwartz pdfs} and the corresponding distributions \defn{Schwartz distributions}

\begin{example}[Schwartz distributions]
  \cref{tab:dens} lists distributions with Schwartz pdfs. \dw{check, in particular logistic}
  \begin{table}
    \begin{center}
    \begin{tabular}{ c|ccc }
     distribution & pdf  & support & parameters\\ \hline
     normal & $\frac 1 {\sigma\sqrt{2\pi}}\exp\left(\frac {-(x-\mu)^2}{2\sigma^2}\right)$ & $\Real$ & $\mu\in\Real, \sigma\in\Realp$\\[3pt]
     half normal & $\frac {\sqrt 2} {\sigma\sqrt{\pi}}\exp\left(\frac {-x^2}{2\sigma^2}\right)$ & $\Realnn$ &  $\sigma\in\Realp$\\[3pt]
     exponential & $\lambda\cdot\exp(-\lambda x)$ & $\Realnn$ & $\lambda\in\Realp$ \\[3pt]
     % gamma & $\frac 1{\Gamma(k)\theta^k}x^{k-1}\exp\left(-\frac x \theta\right)$&$\Realp$& $k,\theta\in\Realp$\\[3pt]
     % Weibull & $\frac k\lambda \left(\frac x\lambda\right)^{k-1}\exp\left(-\frac x\lambda\right)$&$\Realnn$&$\lambda,k\in\Realp$\\[3pt]
     logistic & $\frac {\exp\left(-\frac {x-\mu}{s}\right)}{s\left(1+\exp\left(-\frac {x-\mu}{s}\right)\right)^2}$&$\Real$&$\mu\in\Real, s\in\Realp$
    \end{tabular}
    \end{center}
    \caption{Schwartz distributions and their pdfs}
    \label{tab:dens}
  \end{table}

  Non-examples include the Cauchy distribution and the Gamma distribution.
  The Cauchy distribution famously does not even have an expectation (which would otherwise contradict \cref{lem:Schwprop} below).
  When the shape parameter $k,\alpha<1$ even the pdf itself is unbounded but the Gamma distribution cannot be reparameterised \cite{RTB16b} and therefore it is only of marginal interest for our work regarding the reparametrisation gradient.
\end{example}
We also focus on products of univariate Schwartz functions: if $f_1,\ldots,f_n:\Real\to\Real$ are (univariate) Schwartz functions then $f(x_1,\ldots,x_n)\defeq f_1(x_1)\cdot\cdots\cdot f_n(x_n)$ is a Schwartz function.

We recall some of the pleasing properties of Schwartz functions \dw{add reference}:
\begin{lemma}
  \label{lem:Schwprop}
  Let $f:\Real^n\to\Real$ be a Schwartz function. Then
  \begin{enumerate}
    \item all partial derivatives of $f$ are also Schwartz functions
    \item\label{it:int} $f\in L^p(\Real^n)$; in particular $f$ is integrable: $\int |f(\mathbf x)|\diff\mathbf x<\infty$.
    \item\label{it:prod} if $p:\Real^n\to\Real$ is a polynomial then the product $(f\cdot p):\Real^n\to\Real$ is a Schwartz function.
  \end{enumerate}
\end{lemma}
We conclude with the following which is very important for the present work:
\begin{corollary}[Integrability]
  \label{cor:int}
  Let $f:\Real^n\to\Real$ be a Schwartz function and $g:\Real^n\to\Real$ be such that $|g|$ is bounded by a polynomial. Then $f\cdot g$ is integrable, i.e.\ $\int |f(\mathbf x)\cdot g(\mathbf x)|\diff\mathbf x<\infty$
\end{corollary}



\iffalse
\subsubsection{Tempered Distributions}
A \defn{tempered distribution} (typically denoted by $T$) is a continuous linear functional $\Schwsp(\Real^n)\to\Real$.

Let $f:\Real^n\to\Real$ and suppose $|f|$ is bounded by a polynomial. Then there is a tempered distribution $T_f$ defined by $T_f(g)=\int f\cdot g\diff\lat$.

If $f$ is differentiable, $|f|$ is bounded by a polynomial and $g\in\Schwsp(\Real^n)$
then using integration by parts and \cref{lem:Schwprop} we observe
\begin{align}
  \int \frac{\partial f}{\partial x_j}(\bx)\cdot g(\bx)\diff\bx
  &=\int\underbrace{\left[ f(\bx)\cdot g(\bx)\right]_{-\infty}^\infty}_0\diff\bx_{-j}-\int f(\bx)\cdot\underbrace{\frac{\partial g}{\partial x_j}}_{\text{Schwartz}}(\bx)\diff\bx
  \label{eq:intpart}
\end{align}
This elemtary insight is exploited to stipulate partial derivatives for arbitrary tempered distributions (which may not be of the form $T_f$ for differentiable $f$):
define $\frac{\partial T}{\partial x_j}(g)\defeq-T(\frac{\partial g}{\partial x_j})$.

The property \cref{eq:intpart} will be very useful to show uniform convergence of gradients.
\fi

% \subsection{Quasi Borel Spaces}
\fi

\subsection{Fr\"olicher Spaces}

Fr\"olicher spaces generalise smooth spaces:
%\begin{definition}
  A \emph{Fr\"olicher space} is a triple $(X,\mathcal C_X,\mathcal F_X)$ where
  \begin{enumerate}
    \item $X$ is a set
    \item $\mathcal C_X\subseteq\Set(\Real,X)$ is a set of \emph{curves}
    \item $\mathcal F_X\subseteq\Set(X,\Real)$ is a set of \emph{functionals}
  \end{enumerate}
  satisfying
  \begin{enumerate}
    \item if $c\in\mathcal C_X$ and $f\in\mathcal F_X$ then $f\circ c\in C^\infty(\Real,\Real)$
    \item if $c:\Real\to X$ such that for all $f\in\mathcal F_X$, $f\circ c\in C^\infty(\Real,\Real)$ then $c\in\mathcal C_X$
    \item if $f:X\to\Real$ such that for all $c\in\mathcal C_X$, $f \circ c\in C^\infty(\Real,\Real)$ then $f\in\mathcal F_X$.
  \end{enumerate}
  A \emph{morphism} between Fr\"olicher spaces $(X,\mathcal C_X,\mathcal F_X)$ and $(Y,\mathcal C_Y,\mathcal F_Y)$ is a map $\phi\from X\to Y$ satisfying $f\circ\phi\circ c\in C^\infty(\Real,\Real)$ for all $f\in\mathcal F_Y$ and $c\in\mathcal C_X$.
%\end{definition}

Fr\"olicher spaces and their morphisms constitute a category $\Fr$, which is well-known to be cartesian closed.


==> backup/prop.tex <==
% !TEX root = ../main.tex

\section{Type Soundness: Preconditions for Solving the Optimisation Problem}
\label{sec:prop}

In this section, we establish further installments of type soundness: if a term is (refinement) typable, then it satisfies the basic properties required for an SGD-like solution of the Optimisation \cref{p:opt}, including those discussed in \cref{sec:desiderata}.

%\lo{Point out somewhere which proposition establishes each of (D1) to (D4) (this relates to IMCL22 review criticisms on presentation which we should address).} \lo{Where possible, present these propositions in the same order as (D1) to (D4). Currently they aren't.}




Henceforth, we fix a term-in-context $\para\mid\Sigma\vdash M:\nbt\iota 0 g\Delta$. \dw{Note $e=0$.}


\iffalse
\begin{lemma}
  If $\para,\lat\mid[]\vdash\SFC:\bt\PCFRp 0\Delta$ then $\sup_{(\para,\lat)\in\parasp\times\Real^n}|\sema\SFC(\para,\lat)|<\infty$ for all $0<\eta<1$.
\end{lemma}

\begin{lemma}
If $\para,\lat\mid[]\vdash\SFC:\bt\iota 0\Delta$ then $\sema\SFC$ has this sum form.
If $\para,\lat\mid[]\vdash\SFC:\bt\iota 1\Delta$ then $\sema\SFC$ has this sum form.
\end{lemma}
\fi

\subsection{Integrability, Unbiasedness and Bounded Variance/Hessian}
\label{sec:iuuc}

By \cref{prop:form} $\sem M$ and $\sema M$ (for each $\eta>0$) are bounded by a polynomial. Therefore, by \cref{cor:int}:
\begin{proposition}[Integrability]
  \begin{enumerate}
    \item   $\E\left[\left|\sem M(\para,\lat)\right|\right]<\infty$ for all $\para\in\parasp$.
    \item   $\E\left[\left|\sema M(\para,\lat)\right|\right]<\infty$ for all $\eta>0$ and $\para\in\parasp$.
  \end{enumerate}
\end{proposition}

Each $\sema M$ is clearly differentiable. The following is a consequence of a well-known result about exchanging differentiation and integration, which relies on the dominated convergence theorem \cite[Theorem 6.28]{K13}, see also \cref{app:iuuc}.

\begin{proposition}[Unbiasedness]
  \label{prop:unb}
  For every $\para\in\Real^m$ and $\eta>0$,
  \begin{align*}
    \nabla_\para\E_{\lat}[\sema M(\para,\lat)]=\E_{\lat}[\nabla_\para\sema M(\para,\lat)]
  \end{align*}
  \dw{use notation $\lat\sim\trt$?}
\end{proposition}
As a slight subtlety, for fixed $\eta>0$ we need to bound partial derivatives of $\sema M$ w.r.t.\ $\theta_i$ uniformly.
This is guaranteed by \cref{prop:form}.

By \cref{prop:form}, for each $\eta>0$ even partial derivatives of $\sema M$ up to order 2 can be \emph{uniformly} bounded (in $\para\in\parasp$) by a polynomial. Therefore again by \cref{cor:int}:
\begin{proposition}[Bounded Expectation and Hessian]
  For each $\eta>0$,
  \begin{enumerate}
    \item $\sup_{\para\in\parasp}\E\left[\left|\frac{\partial\sema M}{\partial\theta_i}(\para,\lat)\right|^2\right]<\infty$
    \item $\sup_{\para\in\parasp}\E\left[\left|\frac{\partial^2\sema M}{\partial\theta_i\partial\theta_j}(\para,\lat)\right|\right]<\infty$
  \end{enumerate}
\end{proposition}

As a consequence of the Convergence \cref{prop:csgd}, once an accuracy coefficient $\eta>0$ is fixed, we can employ Stochastic Gradient Descent to find stationary points of $\E_{\lat}[\sem M(\para,\lat)]$:
\begin{theorem}[Convergence on Typable Programs]
  \label{thm:sgdsm}
  Let $\para\mid\trt\vdash M:\nbt\iota 0 g\Delta$ and $\eta>0$.

   Then a SGD sequence $(\para_k)_{k\in\nat}$ for $\sema M$
  % \begin{enumerate}
  %   \item
   is unbounded or
    % \item
     has a \emph{stationary} accumulation point for the $\eta$-smoothed Optimisation \cref{p:optsm}.
  % \end{enumerate}
\end{theorem}

\subsection{Uniform Convergence}

By \cref{prop:form},
$\sema M$ and $\sem M$
are finite sums of functions
\begin{align*}
  (\para,\lat)&\mapsto\left[\rep_\para(\lat)\in V\right]\cdot f(\para,\rep_\para(\lat))\\
  (\para,\lat)&\mapsto\Psi_\eta(\rep_\para(\lat))\cdot f(\para,\rep_\para(\lat))
\end{align*}
where
$\Psi_\eta(\rep_\para(\lat))\sau \left[\rep_\para(\lat)\in V\right]$, $0\leq\Psi_\eta\leq 1$ and $f(\para,\rep_\para(\lat))$ is uniformly bounded by a polynomial $\Real^n\to\Real$.
Therefore, the following is a consequence of \cref{lem:unisau} ($\mdist$ is Schwartz) and linearity:
\begin{proposition}[Uniform Convergence]
  \label{prop:unicon}
  $\E_{\lat\sim\mdist}[\sema M(\para,\lat)]\unif\E_{\lat\sim\mdist}[\sem M(\para,\lat)]$.
\end{proposition}


%
% By \cref{multiplication}:
% \begin{lemma}
%   \label{lem:uniSch}
%   If $\sfun$ is Schwartz, $f_\eta\sau f$ and $g$ uniformly bounded by a polynomial then $\int f_\eta(\para,\lat)\cdot g(\para,\lat)\cdot \sfun(\lat)\diff\lat$ converges uniformly to $\int f(\para,\lat)\cdot g(\para,\lat)\cdot \sfun(\lat)\diff\lat$.
% \end{lemma}

% Note that by \cref{cor:form}, $\sema M\sau\sem M$. Besides, $\E_{\lat\sim\mdist}[f_\eta(\para,\lat)]$ converges to $\E_{\lat\sim\mdist}[f(\para,\lat)]$ uniformly if $f_\eta\sau f$ and  (\cref{lem:unisau}).
% \begin{proposition}[Uniform Convergence]
%   \label{prop:unicon}
%   $\E_{\lat\sim\mdist}[\sema M(\para,\lat)]\unif\E_{\lat\sim\mdist}[\sem M(\para,\lat)]$.
% \end{proposition}


\subsection{Uniform Convergence of the Gradient}
\label{sec:unigrad}

Proving uniform convergence of gradients is more challenging. The main difficulty is that for the (logistic) sigmoid function (cf.~\cref{fig:sig,sec:smoothing}) $\lim_{k\to\infty}\sigma_k'(0)=\infty$ (cf.~\cref{fig:sigd}). Thus, there exist $\para\in\parasp$ and $\lat\in\Real^n$ for which $\nabla_\para\sema M(\para,\lat)$ is unbounded:
\begin{align*}
  \nabla_\theta\sema{\ifc{(\transt\nd {(\lambda z\ldotp z+\theta)})} {\underline 0} {\underline 1}}(\theta,z)=\smooth'(z+\theta)\to\infty
\end{align*}
whenever $\theta=-z$.

Fortunately, this effect again only occurs at ``small'' subsets of the latent space. The key technical trick to taming this behaviour is to cast partial derivatives w.r.t.\ the parameters in terms of gradients w.r.t.\ the latent variables and to use integration by parts, thus eliminating derivatives of $\sigma_k$.

\begin{example}
  \label{ex:unic}
  Recall the term from \cref{ex:form}, which has (smoothed) value functions with 3 summands. To show uniform of the gradients it suffices by linearity of expectation to show uniform convergence of each summand.
  We focus on the second (omitting superscripts):
  \begin{align*}
    \phi_\theta(z)&\defeq c\cdot z+\theta&\Psi_\eta(x)&\defeq \smooth(x)\cdot\smooth(1-x)&f(\theta,x)\defeq\theta
  \end{align*}
  It holds
  \begin{align*}
    &\E_{z\sim\nd}\left[\frac{\partial}{\partial\theta}(\Psi_\eta(\phi_\theta(z)))\cdot f(\theta,\phi_\theta(z))\right]\\
    &=
    \E_{z\sim\nd}\left[\frac{\partial\Psi_\eta\circ\phi_{(-)}}{\partial\theta}(\theta,z)\cdot f(\theta,\phi_\theta(z)\right]+
    \E_{z\sim\nd}\left[\Psi_\eta(\phi_\theta(z)))\cdot \underbrace{\frac{\partial}{\partial\theta}(f(\theta,\phi_\theta(z))}_{=1}\right]
  \end{align*}
  and uniform convergence for the second summand can be shown as for \cref{prop:unicon}.

  By the chain rule we obtain:
  \begin{align}
    \label{eq:extrick}
    \frac{\partial(\Psi_\eta\circ\phi_{(-)})}{\partial\theta}(\theta,z)=\frac 1 c\cdot\frac{\partial(\Psi_\eta\circ\phi_{(-)})}{\partial z}(\theta,z)
  \end{align}
  Note that for this it is essential that the guards (which correspond to the factors in the definition of $\Psi_\eta$) do not depend on the parameters $\theta$, but that they are composed using variables which depend on samples which have been transformed with \emph{one} transformation $\phi_{(-)}$.

  This enables us to employ integration by parts (similarly to \cref{eq:intpart} for derivatives of tempered distributions):
  \begin{align*}
    \E_z\left[\frac{\partial(\Psi_\eta\circ\phi_{(-)})}{\partial\theta}(\theta,z)\right]
    &=\int\nd(z)\cdot\frac 1 c\cdot\frac{\partial(\Psi_\eta\circ\phi_{(-)})}{\partial z}(\theta,z)\diff z\\
    &=\frac 1 c\left([\nd(z)\cdot \Psi_\eta(\phi_\theta(z))]_{-\infty}^\infty+\E_z[z\cdot \Psi_\eta(\phi_\theta(z))]\right)
  \end{align*}
  since $\frac{\partial\nd}{\partial z}(z)=-z\cdot\nd(z)$.
  Due to $0\leq \Psi_\eta(\phi_\theta(z))\leq 1$ the first summand is $0$ and the uniform convergence of the second follows as above.
\end{example}
The reasoning can be generalised by employing inverse Jacobians in \cref{eq:extrick}.
\changed[dw]{For this we exploit the fact that the diffeomorphisms are strong in the sense of \cref{def:sdiffun}.} %, which exist due to the fact that transformations are assumed to be diffeomorphic. %\cref{ex:div} illustrates that the result fails otherwise.
\begin{restatable}[Uniform Convergence of Gradients]{theorem}{unifg}
  \label{prop:unifg}
  Let $\para\mid\trt\vdash M:\nbt\iota 0 g\Delta$. Then
%  If $\parasp\subseteq\Real^m$ is compact then
  \begin{align*}
    \nabla_\para\E_{\lat\sim\msnd}\left[\sema M(\para,\lat)\right]&\unif\nabla_\para\E_{\lat\sim\msnd}\left[\sem M(\para,\lat)\right]&\text{as $\eta\searrow 0$ for $\para\in\parasp$.}
  \end{align*}
\end{restatable}

The significance of \cref{prop:unifg} is that it provides the theoretical basis for obtaining approximately stationary points for the original \cref{p:opt}: given an error tolerance $\epsilon>0$ there exists an accuracy coefficient $\eta>0$ such that $\|\nabla_\para\E_{\lat}[\sema M(\para,\lat)]-\nabla_\para\E_{\lat}[\sem M(\para,\lat)]\|<\epsilon$ for all $\para\in\parasp$. Thus, a stationary point $\para^*\in\parasp$ of the smoothed problem for accuracy coefficient $\eta$ (which thanks to the Convergence \cref{thm:sgdsm} may be obtained by SGD) is approximately stationary:
\begin{align*}
  \|\nabla_\para\E_{\lat\sim\msnd}[\sem M(\para^*,\lat)]\|<\epsilon
\end{align*}
\dw{duplicated}

\iffalse
\subsection{Bounding the Gradient}

\dw{all $|\partial^\alpha\chi_{i,j}|$ are bounded by a poly uniformly in $\para\in\parasp$.}

\begin{lemma}
  \label{lem:boundSch}
  If $\sfun$ is Schwartz, $0\leq\psi_\eta\leq 1$ and $f$ \dw{and partial derivatives} is uniformly bounded by a polynomial then $\sup_{0<\eta<1}\sup_{\para\in\parasp}\int\left|\frac{\partial(\psi_\eta\circ\rep_{(-)})}{\partial\theta_i}(\para,\lat)\cdot f(\para,\lat)\cdot\sfun(\lat)\right|\diff\lat<\infty$.
\end{lemma}




\dw{this holds even for $f_\eta$ if $\E[f_\eta(\para,\lat)]$ uniformly bounded}

\begin{proof}
  We consider partial derivatives w.r.t.\ $z_j$ and employ partial integration:
  \dw{expectation vs.\ integral for $\sfun$}
  \begin{align}
    &\E\left[\left|\frac{\partial(\psi_\eta\circ\rep_{(-)})}{\partial z_j}(\para,\lat)\cdot f(\para,\lat) \right|\right]\notag\\
    &\leq\int [|\psi_\eta(\rep_\para(\lat))\cdot f(\para,\lat)\cdot\pdf_\dist(\lat)|]_{-\infty}^\infty \diff\lat_{-j}+
    \int\left| \psi_\eta(\rep_\para(\lat))\cdot \frac\partial{\partial z_j}\left(f(\para,\lat) \cdot\pdf_\dist(\lat) \right)\right|\diff\lat\notag\\
    &\leq\int\left| \frac{\partial f}{\partial z_j}(\para,\lat) \cdot\pdf_\dist(\lat)\right|\diff\lat+
    \int\left| f(\para,\lat) \cdot \underbrace{\frac{\partial\pdf_\dist}{\partial z_j}}_{\text{Schwartz}}(\lat)\right|\diff\lat
  \end{align}
  \dw{justify absolute value}

  \dw{assumption on $f$, e.g.\ prtial der.\ bounded by poly}

  Next, we consider partial deriavtives w.r.t.\ $\theta_i$:
\begin{align*}
  \E\left[\left|\frac{\partial(\psi_\eta\circ\rep_{(-)})}{\partial\theta_i}(\para,\lat)\cdot f(\para,\lat) \right|\right]
  &\leq\sum_{j=1}^n \E\left[\left|\frac{\partial(\psi_\eta\circ\rep_{(-)})}{\partial z_j}(\para,\lat)\cdot\chi_{i,j}(\para,\lat)\cdot f(\para,\lat) \right|\right]
\end{align*}
and the claim follows from the above reasoning \dw{organisation} because \dw{$\chi_{i,j}$ is bounded by a polynomial}.
\end{proof}

\begin{proposition}
  ...
\end{proposition}
\begin{proof}
  Sufficient to bound a summand.
  \begin{align*}
    \E\left[\left|\frac\partial{\partial\theta_i}\left(\psi_\eta(\rep_\para(\lat))\cdot f(\para,\lat)\right) \right|\right]\leq
    \E\left[\left|\frac{\partial(\psi_\eta\circ\rep_{(-)})}{\partial\theta_i}\cdot f(\para,\lat) \right|\right]+
    \E\left[\left|\psi_\eta(\rep_\para(\lat))\cdot \frac{\partial f}{\partial\theta_i}(\para,\lat) \right|\right]
  \end{align*}
  Uniform boundedness follows from \cref{lem:boundSch,??}, respectively.
\end{proof}

\subsection{Bounding the Hessian}
\begin{lemma}
  If $\sfun$ is Schwartz, $0\leq\psi_\eta\leq 1$ and \dw{also partial derivative bounded} and $f$ \dw{and first two partial derivatives} is uniformly bounded by a polynomial then $\sup_{0<\eta<1}\sup_{\para\in\parasp}\int\left|\frac{\partial^2(\psi_\eta\circ\rep_{(-)})}{\partial\theta_{i'}\partial\theta_i}(\para,\lat)\cdot f(\para,\lat)\cdot\sfun(\lat)\right|\diff\lat<\infty$.
\end{lemma}
Most difficult to bound
\begin{align*}
  &\int\left|\frac{\partial^2(\psi_\eta\circ\rep_{(-)})}{\partial z_j\partial\theta_i}(\para,\lat)\cdot f(\para,\lat)\cdot\sfun(\lat) \right|\diff\lat\\
  &\leq\int \underbrace{\left[\left|\frac{\partial(\psi_\eta\circ\rep_{(-)})}{\partial\theta_i}(\para,\lat)\cdot f(\para,\lat)\cdot\sfun(\lat)\right|\right]_{-\infty}^\infty}_0\diff\lat_{-j}+
  \int\left|\frac{\partial(\psi_\eta\circ\rep_{(-)})}{\partial\theta_i}(\para,\lat)\cdot\frac\partial{\partial z_j}\left(f(\para,\lat)\cdot\sfun(\lat)\right)\right|\diff\lat
\end{align*}
\dw{clarify assumptions}
and this can be bounded by \cref{lem:boundSch}. Besides,
\begin{align*}
  &\int\left|\frac{\partial^2(\psi_\eta\circ\rep_{(-)})}{\partial\theta_{i'}\partial\theta_i}(\para,\lat)\cdot f(\para,\lat)\cdot\sfun(\lat) \right|\diff\lat\\
  &\leq\sum_{j=1}^n\int\left|\frac\partial{\partial\theta_{i'}}\left(\frac{\partial(\psi_\eta\circ\rep_{(-)})}{\partial z_j}(\para,\lat)\cdot\chi_{i,j}(\para,\lat)\right)\cdot f(\para,\lat)\cdot\sfun(\lat) \right|\diff\lat\\
  &\leq\sum_{j=1}^n\int\left|\frac{\partial^2(\psi_\eta\circ\rep_{(-)})}{\partial z_j\partial\theta_{i'}}(\para,\lat)\cdot\chi_{i,j}(\para,\lat)\cdot f(\para,\lat)\cdot\sfun(\lat) \right|\diff\lat\\
  &+
  \sum_{j=1}^n\int\left|\frac{\partial(\psi_\eta\circ\rep_{(-)})}{\partial z_j}(\para,\lat)\cdot\frac{\partial\chi_{i,j}}{\partial\theta_{i'}}(\para,\lat)\cdot f(\para,\lat)\cdot\sfun(\lat) \right|\diff\lat
\end{align*}

\subsection{Bounding the Variance}
\dw{as in ICML}
\fi


==> backup/type.tex <==
% !TEX root = ../main.tex


\subsection{Desiderata}
\label{sec:desiderata}

Given a term-in-context $\para\mid\Sigma\vdash M:\PCFReal$, in order to solve \cref{p:opt}, we desire the following properties:
\begin{enumerate}
  \item \emph{Integrability}: \label{it:int} The objective function of \cref{p:opt} is well-defined: $|\sem M(\para,\lat)$ is integrable, i.e., $\E_{\lat}[|\sem M(\para,\lat)|]<\infty$, for all $\para\in\parasp$.
  \item \emph{Differentiability}: $\E_\lat[\sem M(\para,\lat)]$ is differentiable w.r.t.~$\para$.
  \item \label{it:unbiasedness} \emph{Unbiasedness}: For each $\eta$-smoothing, the Monte Carlo gradient estimator is unbiased:
  \[
    \nabla_\para\E_{\lat}[\sema M(\para,\lat)]=\E_{\lat}[\nabla_\para\sema M(\para,\lat)].
  \]
  \item\label{it:unifgrad} \emph{Uniform Convergence}: $\nabla_\para\E_\lat[\sema M(\para,\lat)]$ converges to $\nabla_\para\E_\lat[\sem M(\para,\lat)]$ uniformly in $\para$.
\end{enumerate}

The significance of Property (\ref{it:unifgrad}) is that it provides a theoretical basis for the construction of approximate stationary points for the original \cref{p:opt}: given an error tolerance $\epsilon>0$ there exists an accuracy coefficient $\eta>0$ such that $\|\nabla_\para\E_{\lat}[\sema M(\para,\lat)]-\nabla_\para\E_{\lat}[\sem M(\para,\lat)]\|<\epsilon$ for all $\para\in\parasp$.
Thus, a stationary point $\para^*\in\parasp$ of the $\eta$-smoothed version of the Problem (which may be obtained by SGD) is approximately stationary for \cref{p:opt}:
\begin{align*}
  \|\nabla_\para\E_{\lat\sim\msnd}[\sem M(\para^*,\lat)]\|<\epsilon
\end{align*}


\subsection{NEW}

\newcommand\ann{\mathfrak a}
\newcommand\sann{\mathfrak b}
\newcommand\mode{\mathfrak p}

Next, we design type systems which establish the desiderata. Typing judgements have the form $\Gamma\mid\trt\vdash_{\mode} M:\tau$, where $\mode$ indicates the property we aim to establish.

To establish properties we also annotate base types. Thus, types are generated from
\begin{align*}
  \trt&::=[z_1\sim\dist_1,\ldots,z_n\sim\dist_n]\\
  \iota&::=\PCFReal\mid\PCFRp\\
  \safet&::=\iota^{\sann}\mid\safet\addtr[]\to\safet\\
  \tau&::=\iota^{\ann}\mid\tau\addtr\trt\to\tau
\end{align*}
where we annotate basetypes and possibly restrict annotations of safe types.

The rules are the same extended with the annotations and property: \dw{order}
\begin{gather*}
  \infer[\Gamma\sqsubseteq\Gamma',\tau\sqsubseteq\tau']{\Gamma'\mid\trt\vdash_{\mode} M:\tau'}{\Gamma\mid\trt\vdash_{\mode} M:\tau}
  \qquad
  \infer{x:\tau \mid [] \vdash_{\mode} x:\tau}{}\\
  \infer{\Gamma\mid[]\vdash_{\mode}\lambda y\ldotp M:\tau_1\addtr\trt\to\tau_2}{\Gamma,y:\tau_1\mid\trt\vdash_{\mode} M:\tau_2}\qquad
  \infer{\Gamma\mid\trt_1\app\trt_2\app\trt_3\vdash_{\mode} M\,N:\tau_2}{\Gamma\mid\trt_2\vdash_{\mode} M:\tau_1\addtr\trt_3\to\tau_2&\Gamma\mid\trt_1\vdash_{\mode} N:\tau_1}\\
  \infer[\mathbf{Para}]{\theta_i:\iota^{\ann}\mid[]\vdash_{\mode}\theta_i:\iota^{\ann}}{}\qquad
  \infer[\mathbf{Const}, r\in\sem\iota]{\mid[]\vdash_{\mode}\underline r:\iota^{\ann}}{}\\
  \infer[\circ\in\{+,\cdot\},\mathbf{Bin}]{\mid[]\vdash_{\mode}\PCFcirc:\iota^{\ann_1}\to\iota^{\ann_2}\to\iota^{\ann}}{}\\
  \infer[\mathbf{Min}]{\mid[]\vdash_{\mode}\PCFmin:\PCFReal^{\ann}\to\PCFReal^{\ann}}{}\qquad
  \infer[\mathbf{Inv}]{\mid[]\vdash_{\mode}\PCFinv:\PCFRp^{\ann}\to\PCFRp^{\ann}}{}\\
  \infer[\mathbf{Exp}]{\mid[]\vdash_{\mode}\PCFexp:\PCFReal^{\ann}\to\PCFRp^{\ann'}}{}\qquad
  \infer[\mathbf{Log}]{\mid[]\vdash_{\mode}\PCFlog:\PCFRp^{\ann}\to\PCFReal^{\ann'}}{}\\
  \infer[\mathbf{If}]{\Gamma\mid\trt\app\trt'\app\trt''\vdash_{\mode}\ifc LMN:\safet}{\Gamma\mid\trt\vdash_{\mode} L:\iota^{\ann}&\Gamma\mid\trt'\vdash_{\mode} M:\safet&\Gamma\mid\trt''\vdash_{\mode} N:\safet}\\
  \infer[\mathbf{Trans}]{\para\mid[z_j\sim\dist]\vdash_{\mode}\transt\dist T:\PCFReal^{\ann}}{\para\mid[]\vdash_{\mode}\sd:\PCFReal^{\ann_1}\to\PCFReal^{\ann_2}}
\end{gather*}

\dw{table with overview}

\subsubsection{Polynomials and Schwartz Distributions}
As a first illustrative step we consider a type system $\vdash_{\mathrm{poly}}$, which restricts terms to polynomials and Schwartz distributions. Integrability follows immediately (\cref{cor:int}).


We need to rule out using $\PCFinv$, $\PCFexp$ and $\PCFlog$ in terms typable $\Gamma\mid\trt\vdash_{\mode} M:\tau$, where $p=\mathbf{t}$. Thus we simply add the (contradictory) side-condition $\mathrm{false}$ in $\mathbf{Inv}$, $\mathbf{Exp}$ and $\mathbf{Log}$.

Besides, in $\mathbf{Trans}$ we require that $\dist$ is a Schwartz distribution.

We do not need to annotate base types (i.e.\ we stipulate $\ann=\ast$).

\begin{proposition}
  If $\para\mid\trt\vdash_{\mathrm{poly}} M:\iota$ then $\sem M$ is a polynomial and all distributions in $\trt$ are Schwartz.
\end{proposition}

\newcommand\ppred{\mathcal P}
To demonstrate this we define a logical predicate $\ppred^{(n)}_\tau$ on $\parasp\times\Real^n\Rightarrow\sem\tau$:
\begin{enumerate}
  \item $f\in\ppred^{(n)}_\iota$ if $f$ is a piecewise polynomial (alternatively: bounded by finitely many polynomials)
  \item $f\in\ppred^{(n)}_{\tau_1\addtr\trt_3\to\tau_2}$ if for all $n_2\in\nat$ and $g\in\ppred^{(n+n_2)}_{\tau_1}$, $f\lrcomp g\in\ppred^{(n+n_2+|\trt_3|)}_{\tau_2}$
\end{enumerate}
where $f:\parasp\times\Real^{n_1}\Rightarrow\sem{\tau_1\addtr\trt_3\to\tau_2}$ and $g:\parasp\times\Real^{n_1+n_2}\Rightarrow\sem{\tau_1}$ define
\begin{align*}
  f\lrcomp g:\parasp\times\Real^{n_1+n_2+|\trt_3|}&\Rightarrow\tau_2\\
  (\para,\tr_1\app\tr_2\app\tr_3)&\mapsto f(\para,\tr_1)(g(\para,\tr_1\app\tr_2),\tr_3)
\end{align*}
\dw{justify well-defined morphisms}

By induction on types it follows:
\begin{lemma}
  \label{lem:ppredcond}
   If $g,h\in\ppred^{(n)}_\tau$ and $f:\parasp\times\Real^n\to\Real$ then $[f(-)<0]\cdot g+[f(-)\geq 0]\cdot h\in\ppred^{(n)}_\tau$.
\end{lemma}

\begin{lemma}[Fundamental]
  If $\para,x_1:\tau_1,\ldots,x_\ell:\tau_\ell\mid\trt\vdash_{\mathrm{poly}} M:\tau$, $n\in\nat$, $\xi^{(1)}\in\ppred^{(n)}_{\tau_1},\ldots,\xi^{(\ell)}\in\ppred^{(n)}_{\tau_\ell}$ then
  $\sem M\flcomp\langle\xi^{(1)},\ldots,\xi^{(\ell)}\rangle\in\ppred^{(n+|\trt|)}_{\tau}$, where
  \begin{align*}
    \sem M\flcomp\langle\xi^{(1)},\ldots,\xi^{(\ell)}\rangle:\parasp\times\Real^{n+|\trt|}&\Rightarrow\sem\tau\\
    (\para,\tr\app\tr')&\mapsto \sem M((\para, \xi^{(1)}(\para,\tr),\ldots,\xi^{(\ell)}(\para,\tr)),\tr')
  \end{align*}
\end{lemma}
\begin{proof}
\begin{enumerate}
  \item For abstractions suppose $\Gamma,x_1:\tau_1,\ldots,x_\ell:\tau_\ell\mid[]\vdash_{\mathrm{poly}}\lambda y\ldotp M:\tau\addtr\trt\to\tau'$ because $\Gamma,x_1:\tau_1,\ldots,x_\ell:\tau_\ell,y:\tau\mid\trt\vdash_{\mathrm{poly}}M:\tau'$.
  To show the claim, suppose $n_2\in\nat$ and $g\in\ppred^{(n+n_2)}_\tau$.
  Call $\widehat\xi^{(i)}$ the extension of $\xi^{(i)}$ to $\parasp\times\Real^{n+n_2}$. By the inductive hypothesis,
  $\sem M\flcomp\langle\xi^{(1)},\ldots,\xi^{(\ell)},g\rangle\in\ppred^{(n+n_2)}_\tau$. Finally it suffices to note that
  \begin{align*}
    \sem M\flcomp\langle\xi^{(1)},\ldots,\xi^{(\ell)}\rangle\lrcomp g=\sem M\flcomp\langle\widehat\xi^{(1)},\ldots,\widehat\xi^{(\ell)},g\rangle
  \end{align*}

  \item For applications it follows immediately from the inductive hypothesis and the definition.
  \item For conditionals we use \cref{lem:ppredcond}.
  \item Next, to show $\sem\PCFcirc\in\ppred^{(0)}_{\iota\to\iota}$ for $\circ\in\{+,\cdot\}$ let $n_1,n_2\in\nat$, $g\in\ppred^{(n_1)}_\iota$, $h\in\ppred^{(n_1+n_2)}_\iota$. Call $\widehat g$ the extension of $g$ to $\parasp\times\Real^{n_1+n_2}\to\sem\iota$.
  Since $\widehat g$ and $h$ are polynomials so is $\widehat g\circ h$. Furthermore clearly,
  \begin{align*}
    \circ\lrcomp g\lrcomp h=\widehat g\circ h
  \end{align*}
  \item The reasoning for $-$ is similar.
  \item For $\mid[\dist]\vdash_{\mathrm{poly}}\sample_\dist$ this is obvious because $\sem\sample=((),[s])\mapsto s$ is clearly a polynomial. \dw{do for transform construct}
  \item $\PCFinv$, $\PCFexp$ and $\PCFlog$ cannot occur.
\end{enumerate}
\end{proof}


\subsubsection{Guard Safety}
type system $\vdash_{\mathrm{gs}}$, annotation of base types $\ann=(\mathfrak S,c)$, where $\mathfrak S$ is a finite set of $z_j$ and $c\in\{\bot,\mathbf{f}\}$.

\dw{track variable depencies first}
\begin{enumerate}
  \item $\mathbf{Para}_2$: $c=\bot$
  \item $\mathbf{Const}_2$: $c=\bot$
  \item $\mathbf{Bin}_2$: $\mathfrak S=\mathfrak S_1\cup\mathfrak S_2$, and $c=\mathbf{f}$ implies $\mathfrak S_1\cap\mathfrak S_2=\emptyset$
  \item All unary operations $\mathbf{Un}$: $\ann=\ann'$
  \item $\mathbf{If}_2$: $c=\mathbf{f}$ \dw{safe type!}
  \item $\mathbf{Trans}_1$: $T$ is strongly diffeomorphic \dw{check}
\end{enumerate}

\subsubsection{Integrability}
Type system $\vdash_{\mathrm{int}}$, base types are annotated by $a\in\{0,1\}$.
\begin{enumerate}
  \item in $\mathbf{Para}$ and $\mathbf{Const}$: $\ann=0$
  \item in $\mathbf{Bin}$: if $\circ=+$ then $\ann=0$
  \item in $\mathbf{Min}$: $\ann=0$
  \item in $\mathbf{Exp}$: $\ann=0$ and $\ann'=1$ \dw{check, make more permissible?}
  \item in $\mathbf{Log}$: $\ann'=1$ \dw{check, make more permissible?}
  \item in $\mathbf{If}$: if $\ann=0$ \dw{also judgements}
  \item $\mathbf{Trans}_4$: $\ann_1=\ann_2=\ann=0$
\end{enumerate}



\dw{1/x?}





\iffalse
\begin{gather*}
  \infer{\theta_i:\nbt\iota 00\emptyset\mid[]\vdash\theta_i:\nbt\iota 00\emptyset}{}\\
  \infer[r\in\sem\iota]{\mid[]\vdash r:\nbt\iota 00\emptyset}{}\\
  % \infer[r\in\Real]{\vdash r:\nbt\PCFReal 00\emptyset}{}\qquad
  % \infer[r\in\Realp]{\vdash r:\nbt\PCFRp 00\emptyset}{}\\
  \infer[\Delta\cap\Delta'=\emptyset\text{ or }g=0]{\mid[]\vdash\PCFplus:\nbt\iota 0g\Delta\to\nbt\iota 0g{\Delta'}\to\nbt\iota 0g{\Delta\cup\Delta'}}{}\\
  \infer[\Delta\cap\Delta'=\emptyset\text{ or }g=0]{\mid[]\vdash\PCFmul:\nbt\iota eg\Delta\to\nbt\iota eg{\Delta'}\to\nbt\iota eg{\Delta\cup\Delta'}}{}\\
  % \infer{\Gamma\mid\trt\app\trt\vdash M\infix\PCFplus M:\nbt\iota 01\Delta}{\Gamma\mid\trt\vdash M:\nbt\iota 01\Delta}\qquad
  % \infer{\Gamma\mid\trt\app\trt\vdash M\infix\PCFmul M:\nbt\iota e1\Delta}{\Gamma\mid\trt\vdash M:\nbt\iota e1\Delta}\\
  \infer[a\in\nat_{>0}]{\Gamma\mid[]\vdash\infix\PCFtimes M:\nbt\iota 01\Delta}{\Gamma\mid[]\vdash M:\nbt\iota 01\Delta}\qquad
  \infer[a\in\nat_{>0}]{\Gamma\mid[]\vdash M\infix\PCFpower:\nbt\iota e1\Delta}{\Gamma\mid[]\vdash M:\nbt\iota e1\Delta}\\
  \infer{\mid[]\vdash\underline-:\nbt\PCFReal 0 g\Delta\to\nbt\PCFReal 0 g\Delta}{}\qquad
  % \infer{\vdash (-)-(-):\nbt\PCFReal 00\Delta\to\nbt\PCFReal 00\Delta\to\nbt\PCFReal 00\Delta}{}\\
  % \infer[\circ\in\{+,\cdot\}]{\vdash\underline\circ:\nbt\iota e0\Delta\to\nbt\iota e0\Delta\to\nbt\iota e0\Delta}{}\\
%  \infer{\vdash\underline+:\nbt\PCFRp eg\Delta\to\nbt\PCFRp eg\Delta\to\nbt\PCFRp eg\Delta}{}\\
  % \infer[\Delta\cap\Delta'=\emptyset]{\vdash\underline+:\nbt\PCFReal e1\Delta\to\nbt\PCFReal e1{\Delta'}\to\nbt\PCFReal e1{\Delta\cup\Delta'}}{}\\
  % \infer[\Delta\cap\Delta'=\emptyset]{\vdash -:\nbt\PCFReal01\Delta\to\nbt\PCFReal 01{\Delta'}\to\nbt\PCFReal0 1{\Delta\cup\Delta'}}{}\\
  \infer{\mid[]\vdash\PCFinv:\nbt\PCFRp e g\Delta\to\nbt\PCFRp eg\Delta}{}\\
  % \infer{ \vdash \PCFexp:\nbt\PCFReal 0g\Delta\to\nbt\PCFRp 1g\Delta}{}\qquad
  % \infer{\vdash \PCFexp:\nbt\PCFReal 0 g\emptyset\to\nbt\PCFRp 0 g\emptyset}{}\\
  \infer[e=1\text{ or }\Delta=\emptyset]{\mid[] \vdash \PCFexp:\nbt\PCFReal eg\Delta\to\nbt\PCFRp eg\Delta}{}\qquad
  \infer{\mid[]\vdash \PCFlog:\nbt\PCFRp e g\Delta\to\nbt\PCFReal 0g\Delta}{}\\
  % \infer[j\in\nat, \sd \text{ strongly diffeomorphic}, \dist\text{ Schwartz}]{\Gamma\mid[\dist]\vdash(\lambda x\ldotp\sd)\,\sample_\dist:\nbt\PCFReal 0 1{\{j\}}}{\Gamma,x:\nbt\PCFReal 00{\{j\}}\mid[]\vdash\sd:\nbt\iota 0 0\Delta}\\
  \infer[\iota=\PCFRp\text{ or }g=1]{\Gamma\mid\trt\app\trt'\app\trt''\vdash\ifc LMN:\safet}{\Gamma\mid\trt\vdash L:\nbt\iota 0g\Delta&\Gamma\mid\trt'\vdash M:\safet&\Gamma\mid\trt''\vdash N:\safet}\\
  \infer[\sd \text{ strongly diffeomorphic}, \dist\text{ Schwartz}]{\para\mid[z_j\sim\dist]\vdash\transt\dist T:\nbt\PCFReal 0 1{\{z_j\}}}{\para\mid[]\vdash\sd:\nbt\PCFReal 00{\{z_j\}}\to\nbt\PCFReal 0 0{\{z_j\}}}\\
\end{gather*}
\fi





\subsection{Discussion of Restrictions}
\label{sec:Discussion of Restrictions}
In order to satisfy the properties of \cref{sec:desiderata},
we need to restrict our programming language of \cref{sec:PL} in a number of ways.

First, observe that integrability (Property (\ref{it:int}) of \cref{sec:desiderata}) can fail:
take $M\equiv(\lambda x\ldotp \PCFexp\,(x\infix\PCFmul x))\,\sample_\nd$: we have $\E_{z\sim\nd}[\sem M(z)]=\infty$, independently of parameters.
Therefore, we aim to ensure that $|\sem M|$ is bounded by a polynomial because that works well with Schwartz densities. \dw{reference}

Furthermore, we need to rule out programs $M$ such that even the expectation of its value semantics is discontinuous (as a function of the parameters).
Take $M\equiv\ifc\theta 0 1$, we have $\E_{\lat}[\sem M(\theta)]=[\theta\geq 0]$ which is discontinuous, let alone differentiable, at $\theta = 0$.
%\changed[lo]{This problematic, because $\E_\lat[\sema M(\theta)]=\sigma_\eta(\theta)$, and so $\E_\lat[\sema M(0)] = 1/2$ for all $\eta$, but $\E_\lat[\sem M(0)]=1$, thus violating \cref{it:unifgrad}.}
Therefore, we require that guards do not depend directly on parameters (but they may do so, indirectly, via a diffeomorphic reparameterisation transform; see \cref{ex:affine transform}).
%\lo{Sure this would rule on the preceding example $M$. However, the reader might reasonably read the preceding example as motivation for requiring the expectation to be continuous in the parameter.}

In order to satisfy Property (\ref{it:unifgrad}) of \cref{sec:desiderata} (Desiderata) we would in particular need $\sema M$ to converge to $\sem M$ \changed[lo]{(for example, because of the product rule of differentiation, in view of Properties (\ref{it:unbiasedness}) and (\ref{it:unifgrad}) of \cref{sec:desiderata})} at least almost everywhere.
This is not so in case
\begin{equation}
  M\equiv\ifc 0 {\theta\cdot\theta}{(\theta-1)\cdot(\theta-1)}.
\label{eq:example guard = 0}
\end{equation}
Notice that the global minimum of $\sem M$ is at $\theta=1$, but that of $\sema M$ is at $\theta=\frac 1 2$, for all $\eta$.
Therefore, we require that guards are non-0 almost everywhere.
%\lo{This condition can also / already be motivated by $M\equiv\ifc\theta 0 1$ (an example considered at the start of \cref{sec:Discussion of Restrictions}).}

%\lo{The following--\cref{ex:div}---would work better after the definition of refinement type system and after introducing the $\transt \dist T$ sugar.}
The following example illustrates why it is \emph{not} sufficient to restrict the term $T$ in the reparameterisation transform, $T \, \sample_\dist$, to (denote) a \emph{bijection} (rather, we require it to be a (strong) diffeomorphism).
\dw{integrate}

%which it is \emph{not} sufficient to restrict terms $\underline\phi_\para(M_1,\ldots,M_\ell,\sample)$ to \emph{bijections}:
\begin{example}[Divergence]
  \label{ex:div}
  Suppose $M\equiv\ifc{((\lambda z\ldotp z\underline{{}^3}\infix\PCFplus\theta)\,\sample_\nd)}{\underline 0}{\underline 1}$. \dw{abuse notation} Let $\phi_\theta(z)\defeq z^3+\theta$.
  Note that despite being bijective, $\phi_\theta\from\Real\to\Real$ is not a diffeomorphism because $\phi^{-1}_\theta(\alpha)=\sqrt[3]{\alpha-\theta}$ is not differentiable at $\alpha=\theta$.
  Then
  \begin{align*}
    \E_{z\sim\nd}[\sem M(\theta,z)]&=\int_{-\sqrt[3]{-\theta}}^\infty\nd(z\mid 0,1)\diff z\\
    \frac\partial{\partial\theta}\E_{z\sim\nd}[\sem M(\theta,z)]&=\frac 1 3\cdot \nd(-\sqrt[3]{-\theta}\mid 0,1)\cdot \theta^{-\frac 2 3}
  \end{align*}
  Therefore $\theta\mapsto\E_{z\sim\nd}[\sem M(\para,z)]$ is not differentiable at $0$. Besides, for $\theta=0$,
  \begin{align*}
    %\E_{z\sim\nd}\left[\frac\partial{\partial\theta}\sema k M(\para,z)\right]=\E_{z\sim\nd}\left[\sigma_k'(z^3)\right]\to\infty
    \E_{z\sim\nd}\left[\frac\partial{\partial\theta}\sema{M(\para,z)} \right]=\E_{z\sim\nd}\left[\sigma_\eta'(z^3)\right]\to\infty
  \end{align*}

\lo{It's plausible that $\E_{z\sim\nd}\left[\sigma_\eta'(z^3)\right]\to\infty$: at 0, the gradient of $\sigma_\eta$ approaches infinity. Is there a simple proof?}
\end{example}

\subsection{Refinement Type System}
We introduce a refinement type system which restricts the terms that are typable w.r.t.~the system of \cref{sec:basic type system}.
Formally, the \emph{refinement types} are generated from the following grammar:
% \lo{Presumably $\alpha_i$ ranges over $x_i$? (and \emph{not} over $\theta_j$).}
% \dw{Yes, they are the sampling variables (from the base distribution) which are then used in the compilation to the simple function calculus. They probably need to be annotated by the distribution to be formal.}
%\newcommand\refbt\rho
\begin{align*}
  &\textbf{trace types}&\trt&::=[z_1\sim\dist_1,\ldots,z_n\sim\dist_n]\\
  &%\textbf{base types}
  &\iota&::=\PCFReal\mid\PCFRp\\
%  &\textbf{refined base types}&\refbt&::=\nbt\PCFReal 0g\Delta\mid\nbt\PCFRp 0g\Delta\mid\nbt\PCFRp 1g\Delta\\
  &\textbf{safe types}&\safet&::=\nbt\PCFReal 0g\Delta\mid\nbt\PCFRp 0g\emptyset&\textit{safe refined base types}\\
  &&&\quad\mid\safet\addtr[]\to\safet&\textit{safe function types}\\
  &\textbf{types}&\tau&::=\nbt\PCFReal 0g\Delta\mid\nbt\PCFRp 0g\emptyset\mid\nbt\PCFRp 1g\Delta&\textit{refined base types}\\
  &&&\quad\mid\tau\addtr\trt\to\tau&\textit{function types}
\end{align*}
%\dw{note: variable annotation in trace type, say more}
%\lo{Need to explain what safe means in ``safe refined base types'' and ``safe function types''. There is a another notion of (guard) safety in \cref{it:guard safe} below.}
where $z_i$ is a variable; $\dist_j$ is a probability distribution that has a Schwartz pdf (denoted $\pdf_{\dist_j}$);
$g \in \{0,1\}$ is a (guard safety) flag;
and $\Delta$ is a finite set of variables $z_j$. \dw{}

The refinement types build on the types of \cref{sec:basic type system}, with two new features which are worth pointing out:
first they are generated from the base types: $\nbt\PCFReal 0g\Delta, \nbt\PCFRp 0g\Delta$ and $\nbt\PCFRp 1 g\Delta$, where $g \in \{0, 1\}$;
secondly, the trace types are now annotated with variables, typically $\Sigma = [z_1\sim\dist_1,\ldots,z_n\sim\dist_n]$ where the variables $z_j$ are pairwise distinct.

\paragraph{The Meaning of $\nbt\iota e g\Delta$}

Intuitively we aim to design a type system such that for a term-in-context, $\para\mid\Sigma\vdash M:\nbt\iota e g\Delta$
\begin{enumerate}
  \item $\log^e \circ \sem M(\para, ({-}))$ is bounded by a polynomial for each $\para \in \Theta$ (recall that by convention $\log^0$ is the identity)
  %if $e=0$ then $|\sem M(\para,(-))|$ is bounded by a polynomial for each $\para\in\parasp$
  %\lo{What about the case of $e = 1$?} \lo{OK. It is discussed in the (type soundness) \cref{prop:form}.}
  \item \label{it:guard safe} if $g=1$ then $M$ is safe to use in guards, in particular
  \begin{enumerate}
    \item\label{it:rep} $\sem M$ only depends on the parameters $\para$ through a diffeomorphism $\rep_\para:\Real^n\to\Real$, i.e.\ $\sem M=\psi\circ\rep_{(-)}$ for some $\psi:\Real^n\to\Real$ \dw{later more restrictions}
    \item $\sem M\neq 0$ a.e.
  \end{enumerate}
  \item $\Delta$ contains identifiers of samples a term may depend on. \dw{vague, state more precisely}
\end{enumerate}




\dw{also independent of $\lat$ for $\PCFRp$ and $e=0$}



% \dw{variables in trace type disjoint}
% where $e\in\{0,1\}$ and $e=1$ implies $\iota=\PCFRp$ and $\Delta\subseteq\{\theta_1,\ldots,\theta_m,\alpha_1,\ldots,\alpha_n\}$.
% \lo{The first clause above should be: $\iota::=\PCFRe \mid \PCFRae$?}
%\lo{I assume we want (environment) $\Gamma = x_1 : \tau_1, \cdots, x_n : \tau_n$ to be finite maps (i.e.~the $x_i$s are pairwise distinct, and $\Gamma$ is a set (of bindings) as opposed to sequence).}

% \dw{$\PCFRae$ is not necessary any more. Whenever we run the risk of not being a.e.\ $\neq 0$, I add $\para$ to $\Delta$ which prevents it from being used in guards. Admittedly that's quite a hack at the moment but I also didn't like $\PCFRae$.}
% where $e \in \nat$ and $\ell \in \nats$ and $\Delta\subseteq\{\theta_1,\ldots,\theta_m,\alpha_1,\ldots,\alpha_n\}$
% and if $\iota$ is $\PCFRae$ then $\theta_i\not\in\Delta$.

% \begin{align*}
%   \PCFRee 0\sqsupseteq\PCFRee 1\sqsupseteq\PCFRee 2\sqsupseteq\cdots
% \end{align*}
% % \dw{better notation than $\addtr$?} \lo{$\addtr$ is definitely better than $\times$}
% and

\newcommand\grt[2]{#1\langle#2\rangle}
\begin{figure}
\begin{framed}
%   \begin{subfigure}{\linewidth}
%   \begin{gather*}
%     \infer[g\geq g',\Delta\subseteq\Delta']{\nbt\PCFReal 0 g\Delta\sqsubseteq\nbt\PCFReal 0{g'}{\Delta'}}{}\qquad
%     \infer[g\geq g']{\nbt\PCFRp 0 g\emptyset\sqsubseteq\nbt\PCFReal 0{g'}{\Delta}}{}\\
%     \infer[g\geq g',\Delta\subseteq\Delta']{\nbt\PCFRp 1 g\Delta\sqsubseteq\nbt\PCFRp 1{g'}{\Delta'}}{}\qquad
%     \infer[g\geq g']{\nbt\PCFRp 0 g\emptyset\sqsubseteq\nbt\PCFRp e{g'}{\Delta}}{}\\
% %    \infer[\iota\sqsubseteq\iota',e\leq e',g\geq g',\Delta\subseteq\Delta']{\nbt\iota eg\Delta\sqsubseteq\nbt{\iota'}{e'}{g'}{\Delta'}}{}\\
%     % \infer{\tau\sqsubseteq\tau}{}\qquad
%       \infer{(\tau_1\addtr\trt\to\tau_2)\sqsubseteq(\tau_1'\addtr\trt\to\tau_2')}{\tau'_1\sqsubseteq\tau_1&
%       \tau_2\sqsubseteq\tau'_2}
%   \end{gather*}
%   \caption{Subtyping}
%   \label{fig:subtypingref}
%   \end{subfigure}

  \begin{subfigure}{\linewidth}
  \begin{gather*}
    \infer[\Gamma\sqsubseteq\Gamma',\tau\sqsubseteq\tau']{\Gamma'\mid\trt\vdash M:\tau'}{\Gamma\mid\trt\vdash M:\tau}
    \qquad
    \infer{x:\tau \mid [] \vdash x:\tau}{}\qquad
    \infer{\theta_i:\nbt\iota 00\emptyset\mid[]\vdash\theta_i:\nbt\iota 00\emptyset}{}\\
    \infer[r\in\sem\iota]{\mid[]\vdash r:\nbt\iota 00\emptyset}{}\\
    \infer[\circ\in\{+,\cdot\},\Delta\cap\Delta'=\emptyset]{\mid[]\vdash_g\PCFcirc:\grt\iota\Delta\to\grt\iota{\Delta'}\to\grt\iota {\Delta\cup\Delta'}}{}\\
    \infer[a\in\nat_{>0}]{\Gamma\mid[]\vdash\infix\PCFtimes M:\nbt\iota 01\Delta}{\Gamma\mid[]\vdash M:\nbt\iota 01\Delta}\qquad
    \infer[a\in\nat_{>0}]{\Gamma\mid[]\vdash M\infix\PCFpower:\nbt\iota e1\Delta}{\Gamma\mid[]\vdash M:\nbt\iota e1\Delta}\\
    \infer{\mid[]\vdash\underline-:\nbt\PCFReal 0 g\Delta\to\nbt\PCFReal 0 g\Delta}{}\qquad
    \infer{\mid[]\vdash\PCFinv:\nbt\PCFRp e g\Delta\to\nbt\PCFRp eg\Delta}{}\\
    \infer[e=1\text{ or }\Delta=\emptyset]{\mid[] \vdash \PCFexp:\nbt\PCFReal eg\Delta\to\nbt\PCFRp eg\Delta}{}\qquad
    \infer{\mid[]\vdash \PCFlog:\nbt\PCFRp e g\Delta\to\nbt\PCFReal 0g\Delta}{}\\
    \infer[\iota=\PCFRp\text{ or }g=1]{\Gamma\mid\trt\app\trt'\app\trt''\vdash\ifc LMN:\safet}{\Gamma\mid\trt\vdash L:\nbt\iota 0g\Delta&\Gamma\mid\trt'\vdash M:\safet&\Gamma\mid\trt''\vdash N:\safet}\\
    \infer[\sd \text{ strongly diffeomorphic}, \dist\text{ Schwartz}]{\para\mid[z_j\sim\dist]\vdash\transt\dist T:\nbt\PCFReal 0 1{\{z_j\}}}{\para\mid[]\vdash\sd:\nbt\PCFReal 00{\{z_j\}}\to\nbt\PCFReal 0 0{\{z_j\}}}\\
    \infer{\Gamma\mid[]\vdash\lambda y\ldotp M:\tau_1\addtr\trt\to\tau_2}{\Gamma,y:\tau_1\mid\trt\vdash M:\tau_2}\qquad
    \infer{\Gamma\mid\trt_1\app\trt_2\app\trt_3\vdash M\,N:\tau_2}{\Gamma\mid\trt_2\vdash M:\tau_1\addtr\trt_3\to\tau_2&\Gamma\mid\trt_1\vdash N:\tau_1}
  \end{gather*}
  \caption{Typing judgments for guards}
  \label{fig:styperef}
\end{subfigure}
  \caption{A Refinement Type System}
\end{framed}
\end{figure}

\begin{figure}
\begin{framed}
  \begin{subfigure}{\linewidth}
  \begin{gather*}
    \infer[g\geq g',\Delta\subseteq\Delta']{\nbt\PCFReal 0 g\Delta\sqsubseteq\nbt\PCFReal 0{g'}{\Delta'}}{}\qquad
    \infer[g\geq g']{\nbt\PCFRp 0 g\emptyset\sqsubseteq\nbt\PCFReal 0{g'}{\Delta}}{}\\
    \infer[g\geq g',\Delta\subseteq\Delta']{\nbt\PCFRp 1 g\Delta\sqsubseteq\nbt\PCFRp 1{g'}{\Delta'}}{}\qquad
    \infer[g\geq g']{\nbt\PCFRp 0 g\emptyset\sqsubseteq\nbt\PCFRp e{g'}{\Delta}}{}\\
%    \infer[\iota\sqsubseteq\iota',e\leq e',g\geq g',\Delta\subseteq\Delta']{\nbt\iota eg\Delta\sqsubseteq\nbt{\iota'}{e'}{g'}{\Delta'}}{}\\
    % \infer{\tau\sqsubseteq\tau}{}\qquad
      \infer{(\tau_1\addtr\trt\to\tau_2)\sqsubseteq(\tau_1'\addtr\trt\to\tau_2')}{\tau'_1\sqsubseteq\tau_1&
      \tau_2\sqsubseteq\tau'_2}
  \end{gather*}
  \caption{Subtyping}
  \label{fig:subtypingref}
  \end{subfigure}

  \begin{subfigure}{\linewidth}
  \begin{gather*}
    %\infer[\Gamma'\sqsubseteq\Gamma,\tau'\sqsubseteq\tau]{\Gamma\mid\trt\vdash M:\tau}{\Gamma'\mid\trt\vdash M:\tau'}
    \infer[\Gamma\sqsubseteq\Gamma',\tau\sqsubseteq\tau']{\Gamma'\mid\trt\vdash M:\tau'}{\Gamma\mid\trt\vdash M:\tau}
    \qquad
    \infer{x:\tau \mid [] \vdash x:\tau}{}\qquad
    \infer{\theta_i:\nbt\iota 00\emptyset\mid[]\vdash\theta_i:\nbt\iota 00\emptyset}{}\\
    \infer[r\in\sem\iota]{\mid[]\vdash r:\nbt\iota 00\emptyset}{}\\
    % \infer[r\in\Real]{\vdash r:\nbt\PCFReal 00\emptyset}{}\qquad
    % \infer[r\in\Realp]{\vdash r:\nbt\PCFRp 00\emptyset}{}\\
    \infer[\Delta\cap\Delta'=\emptyset\text{ or }g=0]{\mid[]\vdash\PCFplus:\nbt\iota 0g\Delta\to\nbt\iota 0g{\Delta'}\to\nbt\iota 0g{\Delta\cup\Delta'}}{}\\
    \infer[\Delta\cap\Delta'=\emptyset\text{ or }g=0]{\mid[]\vdash\PCFmul:\nbt\iota eg\Delta\to\nbt\iota eg{\Delta'}\to\nbt\iota eg{\Delta\cup\Delta'}}{}\\
    % \infer{\Gamma\mid\trt\app\trt\vdash M\infix\PCFplus M:\nbt\iota 01\Delta}{\Gamma\mid\trt\vdash M:\nbt\iota 01\Delta}\qquad
    % \infer{\Gamma\mid\trt\app\trt\vdash M\infix\PCFmul M:\nbt\iota e1\Delta}{\Gamma\mid\trt\vdash M:\nbt\iota e1\Delta}\\
    \infer[a\in\nat_{>0}]{\Gamma\mid[]\vdash\infix\PCFtimes M:\nbt\iota 01\Delta}{\Gamma\mid[]\vdash M:\nbt\iota 01\Delta}\qquad
    \infer[a\in\nat_{>0}]{\Gamma\mid[]\vdash M\infix\PCFpower:\nbt\iota e1\Delta}{\Gamma\mid[]\vdash M:\nbt\iota e1\Delta}\\
    \infer{\mid[]\vdash\underline-:\nbt\PCFReal 0 g\Delta\to\nbt\PCFReal 0 g\Delta}{}\qquad
    % \infer{\vdash (-)-(-):\nbt\PCFReal 00\Delta\to\nbt\PCFReal 00\Delta\to\nbt\PCFReal 00\Delta}{}\\
    % \infer[\circ\in\{+,\cdot\}]{\vdash\underline\circ:\nbt\iota e0\Delta\to\nbt\iota e0\Delta\to\nbt\iota e0\Delta}{}\\
  %  \infer{\vdash\underline+:\nbt\PCFRp eg\Delta\to\nbt\PCFRp eg\Delta\to\nbt\PCFRp eg\Delta}{}\\
    % \infer[\Delta\cap\Delta'=\emptyset]{\vdash\underline+:\nbt\PCFReal e1\Delta\to\nbt\PCFReal e1{\Delta'}\to\nbt\PCFReal e1{\Delta\cup\Delta'}}{}\\
    % \infer[\Delta\cap\Delta'=\emptyset]{\vdash -:\nbt\PCFReal01\Delta\to\nbt\PCFReal 01{\Delta'}\to\nbt\PCFReal0 1{\Delta\cup\Delta'}}{}\\
    \infer{\mid[]\vdash\PCFinv:\nbt\PCFRp e g\Delta\to\nbt\PCFRp eg\Delta}{}\\
    % \infer{ \vdash \PCFexp:\nbt\PCFReal 0g\Delta\to\nbt\PCFRp 1g\Delta}{}\qquad
    % \infer{\vdash \PCFexp:\nbt\PCFReal 0 g\emptyset\to\nbt\PCFRp 0 g\emptyset}{}\\
    \infer[e=1\text{ or }\Delta=\emptyset]{\mid[] \vdash \PCFexp:\nbt\PCFReal eg\Delta\to\nbt\PCFRp eg\Delta}{}\qquad
    \infer{\mid[]\vdash \PCFlog:\nbt\PCFRp e g\Delta\to\nbt\PCFReal 0g\Delta}{}\\
    % \infer[j\in\nat, \sd \text{ strongly diffeomorphic}, \dist\text{ Schwartz}]{\Gamma\mid[\dist]\vdash(\lambda x\ldotp\sd)\,\sample_\dist:\nbt\PCFReal 0 1{\{j\}}}{\Gamma,x:\nbt\PCFReal 00{\{j\}}\mid[]\vdash\sd:\nbt\iota 0 0\Delta}\\
    \infer[\iota=\PCFRp\text{ or }g=1]{\Gamma\mid\trt\app\trt'\app\trt''\vdash\ifc LMN:\safet}{\Gamma\mid\trt\vdash L:\nbt\iota 0g\Delta&\Gamma\mid\trt'\vdash M:\safet&\Gamma\mid\trt''\vdash N:\safet}\\
    \infer[\sd \text{ strongly diffeomorphic}, \dist\text{ Schwartz}]{\para\mid[z_j\sim\dist]\vdash\transt\dist T:\nbt\PCFReal 0 1{\{z_j\}}}{\para\mid[]\vdash\sd:\nbt\PCFReal 00{\{z_j\}}\to\nbt\PCFReal 0 0{\{z_j\}}}\\
    \infer{\Gamma\mid[]\vdash\lambda y\ldotp M:\tau_1\addtr\trt\to\tau_2}{\Gamma,y:\tau_1\mid\trt\vdash M:\tau_2}\qquad
    \infer{\Gamma\mid\trt_1\app\trt_2\app\trt_3\vdash M\,N:\tau_2}{\Gamma\mid\trt_2\vdash M:\tau_1\addtr\trt_3\to\tau_2&\Gamma\mid\trt_1\vdash N:\tau_1}
  %  \infer{\Gamma\mid\trt'\app\trt\vdash M\,N:\tau}{\Gamma\mid\trt\vdash M:\iota\to\tau&\Gamma\mid\trt'\vdash N:\iota}
  \end{gather*}
  \caption{Typing judgments}
  \label{fig:styperef}
\end{subfigure}
  \caption{A Refinement Type System}
\end{framed}
\end{figure}

\dw{PROBLEM in rule for inverses: need to restrict to $\nbt\PCFRp 0 g\emptyset$.}

\dw{safe types in conditionals also means that can't have $\ifc x{\exp z}0$ etc.}

The subtyping relation is presented in \cref{fig:subtypingref}. Intuitively, they capture that we can always drop\footnote{as long as it is not used in guards} guard safety (i.e.\ changing $g$ from $1$ to $0$) and add more depencies to $\Delta$.
% \dw{explain rule for base case: intuitively can drop guard safety flag and add more depencies in $\Delta$. the last rule works because there's no dependence on latent variables} \dw{check}

\dw{say overloading notation}
 \dw{check, other symbol}

In order to enforce condition (\ref{it:rep}) above, we introduce syntactic sugar, $\transt\dist\sd$, for applications of the form $\sd\,\sample_\dist$.
As illustrated in \cref{ex:div}, we further need to restrict the transformation $\sd$:
\begin{definition}
  \label{def:sdiffun}
  A smooth function $\phi_{(-)}:\parasp\times\Real\to\Real$ is \defn{strongly diffeomorphic} if
  \begin{enumerate}
    \item for all $\para\in\parasp$, $\phi_\para:\Real\to\Real$ is a diffeomorphism
    \item\label{it:derb} all partial derivatives of $\phi_{(-)}$ up to order 2 (including $\phi_{(-)}$ itself) are uniformly bounded by a polynomial $\Real\to\Real$
    \item (\emph{Strength}): for every compact $\parasp'\subseteq\parasp$,
    $\inf_{\para\in\parasp'}\inf_{z\in\Real}\left| (\phi_\para)'(z)\right|>0$
  \end{enumerate}
\end{definition}
In particular every affine transformation is a strong diffeomorphism.

\begin{example}[Strength]
A (perhaps contrived) counterexample is $\phi_\theta(z)\defeq \theta^2z+\frac 1 3 \theta^2 z^3-\theta z^2+z$ because $\frac{\partial\phi_\theta}{\partial z}(z)=\theta^2+(\theta z-1)^2$ has no positive lower bound despite being everywhere positive.
\end{example}

We say that a term-in-context, $\para\mid[]\vdash\sd:\nbt\PCFReal 00{\{z_j\}}\to\nbt\PCFReal 0 0{\{z_j\}}$, is \defn{strongly diffeomorphic} if it does not contain conditionals and $\sem\sd$ is a strong diffeomorphism.
Thanks to the absence of conditionals, for all $\para\in\parasp$, $z\in\Real$ and $\eta>0$, $\sema\sd(\para,\etr)(z,\etr)=\sem\sd(\para,\etr)(z,\etr)$ if $\sd$ is strongly diffeomorphic.

\dw{omiting $\Real^0$ due to empty trace}
\dw{Condition (\ref{it:derb}) of \cref{def:sdiffun} automatically holds.}
% \begin{definition}
% \begin{enumerate}
%   \item\label{it:cond} \changed[dw]{$\sd$ does not contain conditionals}
% %  \item $x_1:\bt{\iota_1} 0\emptyset,\ldots,x_\ell:\bt{\iota_\ell} 0\emptyset\mid[]\vdash\sd:\bt\iota 0\Delta$ \lo{flags are missing}
%   \item for all $\para\in\parasp$, $\sem\sd(\para,\etr):\Real\to\Real$ is a diffeomorphism \dw{omiting $\Real^0$ due to empty trace}
%   \item (\emph{Strength}): for every compact $\parasp'\subseteq\parasp$,
%   $\inf_{\para\in\parasp'}\inf_{z\in\Real}\left|\frac {\diff\sem T(\para,[])}{\diff z}(z)\right|>0$
% \end{enumerate}
% \end{definition}



With these ingredients we can define the typing judgments in \cref{fig:styperef}.
%\dw{$\app$ assumes variable annotations are distinct}

\paragraph{Typing Rules: Design and Expressivity}

The refinement type system is based on the basic type system of \cref{sec:basic type system}, and refines it in the sence that if a term-in-context is provable in the refinement type system, then its erasure (i.e.~erasure of the refinements, and the variable annotations of trace types) is provable in the basic type system.
This is straightforward to check.
However a term that is typable in the basic system may not be typable in the refinement system (for example, the term (\ref{eq:guard term 0 long})).

Next we motivate the design of several key typing rules by way of examples.
First we can express affine transformations, in particular, the location-scale transformation using the standard normal as the entropy source (\cref{sec:intro}).

\begin{example}[Affine Transformation]
\label{ex:affine transform}
 % \dw{Can express affine transformations}
Let $\Gamma = \theta_1:\nbt\PCFRp 00\emptyset,\theta_2:\nbt\PCFReal 00\emptyset$.
The following term-in-context is strongly diffeomorphic
\[
  \Gamma \mid [] \vdash \lambda z\ldotp\theta_1\cdot z\mathbin{\underline{+}}\theta_2:\nbt\PCFReal 00{\{z_1\}} \to \nbt\PCFReal 0 0 {\{z_1\}}
\]
(However $\theta_1:\nbt\PCFReal 00\emptyset,\theta_2:\nbt\PCFReal 00\emptyset \mid [] \vdash \lambda z\ldotp\theta_1\cdot z\mathbin{\underline{+}}\theta_2:\nbt\PCFReal 00\emptyset\to\nbt\PCFReal 0 0\Delta$ is \emph{not}.)
Hence, the reparameterisation transform
\[
  G \equiv \Gamma \mid [z_1 : \mathcal D] \vdash  \transt \dist {(\lambda z. \theta_1 \cdot z \mathbin{\underline{+}} \theta_2)} : \nbt \PCFReal 0 1 {\{ z_1 \}}
\]
which has $g$-flag 1, is admissible as a guard term.
Notice that $G$ depends on the parameters, $\theta_1$ and $\theta_2$, \emph{indirectly} through a diffeomorphism, which is permitted by the type system.
%\dw{give the contrived counterexample, where strength fails}
\end{example}

\begin{example}[Non-constant Guards]
  \label{ex:constant function cannot be used in guards}
  We have
  \(
    {}\mid[] \vdash (\lambda x . x \mathbin{\underline{+}} (\PCFmin x)) : \nbt \PCFReal 0 0 {\{z_1\}} \to \nbt\PCFReal 0 0 {\{z_1\}},
  \)
  noting that we must use the $g = 0$ disjunct in the side condition of the $\mathbin{\underline{+}}$ rule; and because $\nbt \PCFReal 0 1 {\{j\}} \sqsubseteq \nbt \PCFReal 0 0 {\{j\}}$, we have
  \[
    {}\mid[] \vdash (\lambda x . x \mathbin{\underline{+}} (\PCFmin x)) : \nbt \PCFReal 0 1 {\{z_1\}} \to \nbt\PCFReal 0 0 {\{z_1\}}.
  \]
  Now $\transt \dist {(\lambda y. y)}$ has type $\nbt \PCFReal 0 1 {\{z_1\}}$ with the $g$-flag necessarily set to 1;
  and so the term
  \[
    M \equiv \big(\lambda x. x\mathbin{\underline{+}}(\PCFmin x)\big) \, \transt \dist {(\lambda y. y)}
  \]
  which denotes 0, has type $\nbt \PCFReal 0 0 {\{z_1\}}$, but \emph{not} $\nbt \PCFReal 0 1 {\{z_1\}}$.
  It follows that $M$ cannot be used in guards (notice the side condition of the rule for conditional), which is as desired: recall Example (\ref{eq:example guard = 0}).
Similarly consider the term
\begin{equation}
N \equiv \big(\lambda x. (\lambda y \, z . \ifc {y \mathbin{\underline{+}} (\PCFmin z)} {M_1} {M_2} ) \, x \, x \big) \,
\transt \dist {(\lambda y. y)}
\label{eq:guard term 0 long}
\end{equation}
When evaluated, the term ${y \mathbin{\underline{+}} (\PCFmin z)}$ in the guard has denotation 0.
For the same reason as above, the term $N$ is not refinement typable.
\end{example}

\iffalse
It is straightforward:
\begin{lemma}
  If $\Gamma\mid[\dist_1,\ldots,\dist_n]\vdash M:\tau$ then all $\dist_i$ are Schwartz.
\end{lemma}
\fi

\dw{check that second rule for exp works everywhere}
\dw{conditional}
\dw{check inverse rule}


% \begin{restatable}[Substitution]{lemma}{subst}
%   \label{lem:subst}
%   If $\Gamma,x:\tau'\mid\trt\vdash M:\tau$ and $\Gamma\mid[]\vdash N:\tau'$ then $\Gamma\mid\trt\vdash M[N/x]:\tau$.
%   % \lo{TYPO: Should be $\sem M((\gamma,\sem V(\gamma, [])),\lat)=\sem{M[V/x]}(\gamma,\lat)$.}
% \end{restatable}

%\paragraph{Expressivity}
\dw{can deal with log densities as arising in variational inference. could make type system more complicated, future work}
\dw{can't deal with $\ifc{\PCFlog\, 2}MN$}
\dw{comment on incompleteness, especially to detect piecewise non-constant analyticity}
\dw{in particular affine guards can be typed}
\dw{\emph{strong} diffeomorphism needed?}

The type system is however incomplete, in the sense that there are terms-in-context that satisfy the properties of \cref{sec:desiderata} (Desiderata) but which are not typable.

\begin{example}[Incompleteness] The following term-in-context denotes the ``identity'':
\[
  {}\mid[] \vdash (\lambda x . (\underline{2} \cdot x) \mathbin{\underline{+}} (\PCFmin x)) : \nbt \PCFReal 0 1 {\{z_1\}} \to \nbt\PCFReal 0 0 {\{z_1\}}
\]
but it does \emph{not} have type $\nbt \PCFReal 0 1 {\{z_1\}} \to \nbt\PCFReal 0 1 {\{z_1\}}$.
Then, using the same reasoning as \cref{ex:constant function cannot be used in guards}, the term
\[
  G \equiv (\lambda x. (\underline{2} \cdot x) \mathbin{\underline{+}} (\PCFmin x)) \, \transt \dist {(\lambda y. y)}
\]
has type $\nbt \PCFReal 0 0 {\{z_1\}}$, but \emph{not} $\nbt \PCFReal 0 1 {\{z_1\}}$, and so $\ifc G 0 1$ is not typable, even though $G$ can safely be used in guards.
\end{example}

\begin{example}[Encoding the ELBO for Variational Inference]
  Finally, we illustrate that our type system can be used to express value functions the expectation of which is the ELBO for variational inference.

  First, we define a term for the pdf of normals with mean $m$ and standard derivation $s$:
  \begin{align*}
    N\equiv \lambda x,m,s\ldotp \big(\underline{\sqrt{2\pi}}\infix\PCFmul s)\PCFinv\infix\PCFmul\PCFexp\,(\underline{-0.5}\infix\PCFmul(z\infix\PCFplus(\PCFmin m))\cdot s\PCFinv\big)\underline{{}^2}
  \end{align*}
  Note that $\mid[]\vdash N:\nbt\PCFReal 0 0{\{z_1\}}\to\nbt\PCFReal 0 0\emptyset\to\nbt\PCFRp 0 0\emptyset\to\nbt\PCFRp 1 0{\{z_1\}}$.


  We consider the example considered by \cite{LYY18} in their Prop.~2 to prove the biasedness of the reparametrisation gradient. (In \cref{ex:biased} we discussed a simplified version thereof.)
  The joint density is
  \begin{align*}
    p(\alpha)&\defeq \nd(\alpha\mid 0,1)\cdot
    \begin{cases}
      \nd(0\mid -2,1)&\tif\alpha<0\\
      \nd(0\mid 5,1)&\tow
    \end{cases}
  \end{align*}
  and they use a variational family with density $q_\theta(\alpha)\defeq\nd(\alpha\mid \theta,1)$, which is reparametrised using a standard normal noise distribution and transformation $z\mapsto z+\theta$.

  Finally, we can define
  \begin{align*}
    M&\equiv \big(\lambda \alpha_1\ldotp \underbrace{\PCFlog\,(N\,\alpha_1\,0\,1)+\ifc {\alpha_1}{\PCFlog\,(N\,\underline 0\,\underline{-2}\,{\underline 1})}{\PCFlog\,(N\,\underline 0\,\underline 5\,\underline 1)}}_{\log p}-\underbrace{\PCFlog\,(N\,\alpha_1\,\theta\,\underline 1)}_{\log q_\theta}\big)\\
    &\hspace*{6cm}\,\big(\transt\nd (\lambda z_1\ldotp z_1+\theta)\big)
  \end{align*}
  Note that $\theta:\nbt\PCFReal 0 0\emptyset\mid[z_1\sim\nd]\vdash M:\nbt\PCFReal 0 0{\{z_1\}}$.
\end{example}

\section{Decomposition to Canonical Forms}
\label{sec:type soundness}

In this section we establish that
typable terms of base types have a canonical form (\cref{prop:form}), a property which we use heavily in \cref{sec:prop} to establish the pleasing properties related to the reparametrisation gradient estimator and stochastic gradient descent.

Henceforth, we fix parameters $\theta_1:\nbt{\iota_1}00\emptyset,\ldots,\theta_m:\nbt{\iota_m}00\emptyset$.
\begin{assumption}
  \label{ass:comp}
  We assume that $\parasp\subseteq\sem{\iota_1}\times\cdots\times\sem{\iota_m}$, is compact.
\end{assumption}
\begin{assumption}
  \label{ass:sig}
  For every $\delta>0$, $\smooth\unif[(-)>0]$ on $(-\infty,-\delta)\cup(\delta,\infty)$.

  For every $\eta>0$, $\sup_{x\in\Real}|\smooth'(x)|,\sup_{x\in\Real}|\smooth''(x)|<\infty$
\end{assumption}
\dw{why not indented and numbered separately?}

\dw{connections to dirac delta}
Note that e.g.\ the logistic sigmoid satisfies \cref{ass:sig}.





% \lo{We should give $f_\eta\sau f$ a name in English. I think ``almost uniform convergence'' is appropriate. The snag is that there is already a notion of almost uniform convergence in the literature, but that assumes countable sequences of functions $f_k$ with $k \in \nat$. I would propose that we present $f_\eta\sau f$ as the natural extension, of same underlying notion, to uncountable sequences $f_\eta$ where $\eta \in (0, \infty)$.}
%
%
% \lo{OK. The notion $f_\eta\sau f$ is important to the convergence theorem. We should include (perhaps as a remark) the preceding points, motivating the definition and relating it to ``almost uniform convergence'' in the literature.}


Now, we address Property (\ref{it:unifgrad}) of \cref{sec:desiderata} (Desiderata), i.e.\ how to show that for $\para\mid\trt\vdash M:\nbt\iota 0 g\Delta$, the $\eta$-smoothed %$\E[\sem M(\para,\lat)]$ converges to
$\E[\sema M(\para,\lat)]$ converges uniformly for $\para\in\parasp$ as $\eta\searrow 0$. It would be sufficient to prove that $\sema M$ converges to $\sem M$ uniformly in both $\para$ and $\lat$. Unfortunately, this does \emph{not} hold:
\begin{example}
  \label{ex:nconv}
  Observe that
  \begin{align*}
    f(\theta,z)\defeq\sem{\ifc{(\transt\nd(\lambda z\ldotp z\mathbin{\underline{+}}\theta))}{0}{1}}(\theta,z)=[z\mathbin{\underline{+}}\theta\geq 0]
  \end{align*} is discontinuous at $(\theta,-\theta)$.
  Therefore, despite the fact that
  \begin{align*}
    f_\eta(\theta,z)\defeq\sema{\ifc{(\transt\nd(\lambda z\ldotp z+\theta))}{0}{1}}(\theta,z)=\smooth(z\mathbin{\underline{+}}\theta)
  \end{align*}
  converges a.e.\ to $f$, the convergence cannot possibly be uniform.
\end{example}
However, \changed[lo]{if $\para\mid\Sigma\vdash M:\nbt\iota 0 g\Delta$ then} $\sema M$ \emph{does} converge to $\sem M$ %in a sense doubly-(almost) uniformly:
uniformly almost uniformly, i.e.,
uniformly in $\para\in\parasp$ and \emph{almost} uniformly in $\lat\in\Real^n$. Formally, we define:
\begin{definition}
  Let $f,f_\eta:\parasp\times \Real^n\to\Real$, $\mu$ be a \dw{what} measure on $\Real^n$.
  We say that $f_\eta$ \defn{converges uniformly almost uniformly} to $f$ (notation: $f_\eta\sau f$) if there exist sequences $(\delta_k)_{k\in\nat}$, $(\epsilon_k)_{k\in\nat}$ and $(\eta_k)_{k\in\nat}$ such that $\lim_{k \to \infty}\delta_k=0=\lim_{k \to \infty}\epsilon_k$; and for every $k\in\nat$ and $\para\in\parasp$ there exists $U\subseteq \Real^n$ such that
  \begin{enumerate}
    \item $\mu(U)<\delta_k$ and
    \item for every $0<\eta<\eta_k$ and $\lat\in\Real^n\setminus U$, $|f_\eta(\para,\lat)-f(\para,\lat)|<\epsilon_k$.
  \end{enumerate}
\lo{Though the definition does not require it, in this paper's use case ($\eta$ being the accuracy coefficient), it is the case that $\lim_{k \to \infty}\eta_k = 0$.}
\dw{Intuitively, typically we need to make $\eta_k$ small to obtain Item 2.}
\end{definition}
If $f,f_\eta$ are independent of $\para$ this notion coincides with standard almost uniform convergence.
\dw{add reference}


\lo{Rephrasing of $f_\eta\sau f$ on $V$: For every $\{\epsilon_k\}_k$ with $\lim\epsilon_k = 0$, there exist $\{\eta_k\}_k$, $\{U_{k,\para} \subseteq V\}_{k, \para}$ and $\{\delta_k\}_k$ with $\lim\delta_k = 0$, such that for every $k$ and $\para$, $\mu(U_{k,\para})<\delta_k$, and for every $0<\eta<\eta_k$ and $\lat\in\Real^n\setminus U_{k,\para}$, $|f_\eta(\lat)-f(\lat)|<\epsilon_k$.}


  % \item $f\in\pred_{n,\tau_1\addtr\trt\to\tau_2}$  if for all $n'$ and $g\in\pred_{n',\tau_1}$,
  % $h\in\pred_{n\mathbin{\underline{+}}|\trt|\mathbin{\underline{+}}n',\tau_2}$, where $h(\para,\tr_1\app\tr_2\app\tr_3)\defeq f(\para,\tr_1)(g(\para,\tr_2),\tr_3)$ \dw{justify morphism}
% \end{enumerate}ad

Recall $f_\eta(\theta,z)=\smooth(z\mathbin{\underline{+}}\theta)$ and $f(\theta,z)= [z\mathbin{\underline{+}}\theta\geq 0]$ from \cref{ex:nconv}.
It holds that $f_\eta\sau f$. \dw{add justification}
Thus, this weaker form of convergence holds although uniform convergence fails.

\lo{NOTATION: Should mention use of the Iverson Bracket $[\phi]$ for predicate $\phi$.}

Uniform almost uniform convergence entails uniform convergence of expectations:
\begin{lemma}
  \label{lem:unisau}
  If each $f,f_\eta:\parasp\times\Real^n\to[0,1]$, $f_\eta\sau f$, $g$ is uniformly (in $\para\in\parasp$) bounded by a polynomial and $\mdist$ is Schwartz.

  Then $\E_{\lat\sim\mdist}[f_\eta(\para,\lat)\cdot g(\para,\lat)]$ converges to $\E_{\lat\sim\mdist}[f(\para,\lat)\cdot g(\para,\lat)]$ uniformly in $\para\in\parasp$.
\end{lemma}
\begin{proof}
  By \cref{cor:int}, $\E_{\lat\sim\mdist}[|g(\para,\lat)|^2]$ is bounded. Therefore, by the Cauchy-Schwartz inequality it suffices to show the uniform convergence of $\E_{\lat\sim\mdist}[|f_\eta(\para,\lat)-f(\para,\lat)|^2]$ to $0$.

  Let $\epsilon>0$. By uniform almost uniform convergence of $f_\eta$ to $f$ there exists $k$ such that $\delta_k,\epsilon_k<\frac\epsilon 2$.

  Suppose $\para\in\parasp$ and $\eta<\eta_k$.
  Let $U\subseteq\Real^n$ be the witness for almost uniform convergence of $f_\eta$, $k$ and $\para$. In particular,
  $\E_{\lat\sim\mdist}[[\lat\in U]]<\delta_k<\frac\epsilon 2$ and for every $\lat\in\Real^n\setminus U$, $|f_\eta(\para,\lat)-f(\para,\lat)|<\epsilon_k<\frac\epsilon 2$.

% Cauchy-Schwartz:
% \begin{align*}
%   &\left|\E_{\lat\sim\mdist}[f_\eta(\para,\lat)]-\E_{\lat\sim\mdist}[f(\para,\lat)]\right|\\
%   &\leq\left|\E_{\lat\sim\mdist}[f_\eta(\para,\lat)\cdot g(\para,\lat)]-\E_{\lat\sim\mdist}[f(\para,\lat)\cdot g(\para,\lat)]\right|\\
%   &\leq\sqrt{\E_{\lat\sim\mdist}\left[\left|f_\eta(\para,\lat)-f(\para,\lat)\right|^2\right]}\cdot\sqrt{\E_{\lat\sim\mdist}\left[\left|g(\para,\lat)\right|^2\right]}
% \end{align*}

  \begin{align*}
    % &\left|\E_{\lat\sim\mdist}[f_\eta(\para,\lat)\cdot g(\para,\lat)]-\E_{\lat\sim\mdist}[f(\para,\lat)\cdot g(\para,\lat)]\right|\\
    &\E_{\lat\sim\mdist}[|f_\eta(\para,\lat)-f(\para,\lat)|^2]\\
    &\leq\E_{\lat\sim\mdist}\left[[\lat\in U]\cdot|f_\eta(\para,\lat)-f(\para,\lat)|^2\right]+\E_{\lat\sim\mdist}\left[[\lat\in\Real^n\setminus U]\cdot|f_\eta(\para,\lat)-f(\para,\lat)|^2\right]\\
    &\leq\E_{\lat\sim\mdist}\left[[\lat\in U]\right]+\E_{\lat\sim\mdist}\left[[\lat\in\Real^n\setminus U]\cdot\frac{\epsilon}{2}\right]\\
    &\leq\epsilon
    %\qedhere READD
  \end{align*}
  % \begin{align*}
  %   &\left|\E_{\lat\sim\mdist}[f_\eta(\para,\lat)\cdot g(\para,\lat)]-\E_{\lat\sim\mdist}[f(\para,\lat)\cdot g(\para,\lat)]\right|\\
  %   &\leq\E_{\lat\sim\mdist}\left[[\lat\in U]\cdot|f_\eta(\para,\lat)-f(\para,\lat)|\cdot|g(\para,\lat)|\right]+\E_{\lat\sim\mdist}\left[[\lat\in\Real^n\setminus U]\cdot|f_\eta(\para,\lat)-f(\para,\lat)|\cdot|g(\para,\lat)|\right]\\
  %   &\leq
  % \end{align*}
\end{proof}

Finally, we need to aggregate the effect of transformations of multiple samples. Therefore, we define:
\begin{definition}
  \label{def:sdiffmul}
  A function $\rep_{(-)}:\parasp\times\Real^n\to\Real^n$ is \defn{strongly diffeomorphic} if there exist strong diffeomorphisms $\phi^{(1)}_{(-)},\ldots,\phi^{(n)}_{(-)}:\parasp\times\Real\to\Real$ in the sense of \cref{def:sdiffun} such that
  $(\rep_\para(\lat))_j=\phi^{(j)}_\para(z_j)$, i.e.\ the $j$-th entry is obtained using the $j$-th diffeomorphism.
\end{definition}

Having posited the relevant notions we can state:
\lo{PRESENTATION: In this proposition, I would use the indicator function in place of $\Psi^{(k)}$, and $\sigma_\eta$ in place of $\Psi^{(k)}_\eta$ (thus making it significantly more readable and comprehensible!), and then say in a remark that they can be generalised.}
\dw{the problem is that it's more complex than that due to products, nesting etc.\ but I'll think about it}

\dw{Intuition!!!}

\begin{restatable}[Decomposition to Canonical Forms]{proposition}{form}
  \label{prop:form}
  Let $\para\mid[z_1 \sim \dist_1,\ldots, z_n \sim \dist_n]\vdash M:\nbt\iota e g\Delta$.
  Then there exist $\ell\in\nat$, $\rep_{(-)}$, $V^{(k)}\subseteq\Real^n$, $\Psi_\eta^{(k)}:\Real^n\to[0,1]$,
  % $\bowtie^{(k)}\in {\{<,\geq\}}$,
   $f^{(k)}:\parasp\times\Real^n\to\sem\iota$ (for $1\leq k\leq\ell$ and $\ell\in\Realp$) satisfying
  \begin{align}
    \label{eq:form}
    \log^e\left(\sem M(\para,\lat)\right)&=\sum_{k=1}^\ell \left[\rep_\para(\lat)\in V^{(k)}\right]\cdot f^{(k)}(\para,\rep_\para(\lat))\\
    \label{eq:formsmooth}
    \log^e\left(\sema M(\para,\lat)\right)&=\sum_{k=1}^\ell \Psi_\eta^{(k)}(\rep_\para(\lat))\cdot f^{(k)}(\para,\rep_\para(\lat))
  \end{align}
  where
  \begin{enumerate}
    \item $\rep_{(-)}$ is a strong diffeomorphism (cf.~\cref{def:sdiffmul})
    \item for each $\eta>0$, the partial derivatives up to order $2$ of each $\Psi_\eta^{(k)}$ are bounded by a polynomial $\Real^n\to\Real$
%    \item \changed[dw]{partial derivates of each $\Psi_\eta^{(k)}$ up to order $2$ are uniformly integrable} \dw{is previous item redundant?}
    \item The $V^{(k)}$ form a partition of $\Real^n$ and $\E[[\lat\in\boundary V^{(k)}]]=0$
    \item $\Psi_\eta^{(k)}\circ\rep_{(-)}\sau[\rep_{(-)}\in V^{(k)}]$
    % \dw{need: $\Psi^{(k)}\neq 0$ a.e. and it is analytic?}
%    \item $(\para,\lat)\mapsto f^{(k)}(\para,\rep_\eta(\para,\lat))\sau (\para,\lat)\mapsto f^{(k)}(\para,\rep(\para,\lat))$
    \item $f^{(k)}$ is analytic and partial derivatives up to order 2 (incl.\ $f^{(k)}$ itself) are uniformly (in $\para\in\parasp$) bounded by a polynomial $\Real^n\to\Real$
    \item\label{it:delta} $f^{(k)}$ only depends on $\alpha_j$ if $z_j\in\Delta$ \dw{$\alpha_j$ is transformed $z_j$}
    \item\label{it:nc} if $g=1$ then $f^{(k)}$ is not constant and does not depend on the parameters $\para$ \dw{clarify}
  \end{enumerate}
\end{restatable}
  In the above we mean $\log^0=\mathrm{id}$ and $\log^1=\log$.

Intuitively, each summand corresponds to a branch of the execution, the $V^{(k)}$ capture the constraints on the transformed samples and the $f^{(k)}$ define the value-function in each branch. The $\Psi^{(k)}$ are products of $\smooth$s capturing the smoothing of the discontinuity arising due to $[\rep_\para(\lat)\in V^{(k)}]$.

\cref{prop:form} can be proved using a logical relations approach (see \cref{app:can}) between smoothed $\parasp\times\Real^n\Rightarrow\sema\tau$ and measurable $\parasp\times\Real^n\Rightarrow\sem\tau$.
\dw{explain more why the properties hold, give proof sketch}
  \begin{example}
    \label{ex:form}
    Consider the (typable) term $M$ defined by
   \begin{align*}
     \sd&\equiv\lambda z\ldotp \underline c\infix\PCFmul z\infix\PCFplus\theta\\
     M&\equiv(\lambda x\ldotp (\ifc x{x\infix\PCFmul x}{(\ifc{x\infix\PCFplus(\underline {-1})}{\theta}{\underline 0})})\;
     (\transt\nd\sd)
   \end{align*}
   where $0\neq c\in\Real$ is a constant. Note that $\nbt\PCFReal 0 0\emptyset\mid[z_1\sim\nd]\vdash M:\nbt\PCFReal 0 0{\{z_1\}}$.
   Let
   \begin{align*}
     \phi_\theta(z)&\defeq c\cdot z+\theta\\
     V^{(1)}&\defeq(-\infty,0)& \Psi^{(1)}(x)&\defeq \smooth(-x)&f^{(1)}(\theta,x)\defeq x^2\\
     V^{(2)}&\defeq[0,\infty)\cap(-\infty,1)&\Psi^{(2)}(x)&\defeq \smooth(x)\cdot\smooth(1-x)&f^{(2)}(\theta,x)\defeq\theta\\
     V^{(3)}&\defeq [0,\infty)\cap[1,\infty)&\Psi^{(3)}(x)&\defeq \smooth(x)\cdot\smooth(x-1)&f^{(3)}(\theta,x)\defeq0
   \end{align*}
   We have
   \begin{align*}
     \sem M(\theta,z)&= \sum_{k=1}^3[\phi_\theta(z)\in V^{(k)}]\cdot f^{(k)}(\theta,\phi_\theta(z))&
     \sema M(\theta,z)&= \sum_{k=1}^3 \Psi^{(k)}(\phi_\eta(z))\cdot f^{(k)}(\theta,\phi_\theta(z))
   \end{align*}
   \dw{check}
  \end{example}


==> backup/type2.tex <==
% !TEX root = ../main.tex

Next, we aim to restrict the language to fragments which have desirable properties.
In this section, we aim to establish the well-definedness of the optimisation problem and the convergence of SGD for fixed accuracy coefficient (the latter includes unbiasedness of the reparametrisation gradient estimator, cf.~\cref{prop:csgd}). In \cref{??} we focus on uniform convergence of the problem.

Our approach is based on a generic type system to establish various properties.

Typing judgements have the form $\Gamma\mid\trt\genj M:\tau$, where $?$ indicates the property we aim to establish.

To establish properties we also annotate base types. Thus, types are generated from
\begin{align*}
  \trt&::=[z_1\sim\dist_1,\ldots,z_n\sim\dist_n]\\
  \iota&::=\PCFReal\mid\PCFRp\\
  \safet&::=\iota^{\sann}\mid\safet\addtr[]\to\safet\\
  \tau&::=\iota^{\ann}\mid\tau\addtr\trt\to\tau
\end{align*}
where we annotate basetypes and possibly restrict annotations of safe types.

The rules are the same extended with the annotations and property: \dw{order}
\begin{gather*}
  \infer[\Gamma\sqsubseteq\Gamma',\tau\sqsubseteq\tau']{\Gamma'\mid\trt\genj M:\tau'}{\Gamma\mid\trt\genj M:\tau}
  \qquad
  \infer{x:\tau \mid [] \genj x:\tau}{}\\
  \infer{\Gamma\mid[]\genj\lambda y\ldotp M:\tau_1\addtr\trt\to\tau_2}{\Gamma,y:\tau_1\mid\trt\genj M:\tau_2}\qquad
  \infer{\Gamma\mid\trt_1\app\trt_2\app\trt_3\genj M\,N:\tau_2}{\Gamma\mid\trt_2\genj M:\tau_1\addtr\trt_3\to\tau_2&\Gamma\mid\trt_1\genj N:\tau_1}\\
  \infer[\mathbf{Para}]{\theta_i:\iota^{\ann}\mid[]\genj\theta_i:\iota^{\ann}}{}\qquad
  \infer[\mathbf{Const}, r\in\sem\iota]{\mid[]\genj\underline r:\iota^{\ann}}{}\\
  \infer[\circ\in\{+,\cdot\},\mathbf{Bin}]{\mid[]\genj\PCFcirc:\iota^{\ann_1}\to\iota^{\ann_2}\to\iota^{\ann}}{}\\
  \infer[\mathbf{Min}]{\mid[]\genj\PCFmin:\PCFReal^{\ann}\to\PCFReal^{\ann}}{}\qquad
  \infer[\mathbf{Inv}]{\mid[]\genj\PCFinv:\PCFRp^{\ann}\to\PCFRp^{\ann}}{}\\
  \infer[\mathbf{Exp}]{\mid[]\genj\PCFexp:\PCFReal^{\ann}\to\PCFRp^{\ann'}}{}\qquad
  \infer[\mathbf{Log}]{\mid[]\genj\PCFlog:\PCFRp^{\ann}\to\PCFReal^{\ann'}}{}\\
  \infer[\mathbf{If}]{\Gamma\mid\trt\app\trt'\app\trt''\genj\ifc LMN:\safet}{\Gamma\mid\trt\genj L:\iota^{\ann}&\Gamma\mid\trt'\genj M:\safet&\Gamma\mid\trt''\genj N:\safet}\\
  \infer[\mathbf{Sample}]{\mid[z_j\sim\dist]\genj\sample_\dist:\PCFReal^{\ann}}{}
\end{gather*}

\begin{table}[ht]
  \caption{foo bar, explain $\dep$}
  \label{tab:type}
  \centering
  \small
  \begin{tabular}{llcc}
    \toprule
    property & Section & judgement & annotation  \\
    \midrule
    well-definedness & \cref{sec:basic type system} & $\vdash$ & -- \\
    \multirow{2}{*}{correctness SGD} & \cref{sec:poly}  & $\polyj$ & none/$\ast$  \\
    & \cref{sec:int} & $\intj$ & $0/1$\\
    uniform convergence & \cref{sec:gs} & $\gsj$ & $(\bot,\dep)/(\true,\dep)$ \\
    \bottomrule
  \end{tabular}

\end{table}

\dw{state trivial property that types can be erased}


==> sections/fixed.tex <==
% !TEX root = ../main.tex


==> sections/sem.tex <==
% !TEX root = ../main.tex

We define a denotational approximation semantics $\sema\eta\cdot$ (for $\eta>0$) based on the CCC of Fr\"olicher spaces.
\subsection{Fr\"olicher Spaces}
Recall the definition of Fr\"olicher spaces:
\begin{definition}
  A \emph{Fr\"olicher space} is a triple $(X,\mathcal C_X,\mathcal F_X)$ where
  \begin{enumerate}
    \item $X$ is a set
    \item $\mathcal C_X\subseteq\Set(\Real,X)$ is a set of \emph{curves}
    \item $\mathcal F_X\subseteq\Set(X,\Real)$ is a set of \emph{functionals}
  \end{enumerate}
  satisfying
  \begin{enumerate}
    \item if $c\in\mathcal C_X$ and $f\in\mathcal F_X$ then $f\circ c\in C^\infty(\Real,\Real)$
    \item if $c:\Real\to X$ such that for all $f\in\mathcal F_X$, $f\circ c\in C^\infty(\Real,\Real)$ then $c\in\mathcal C_X$
    \item if $f:X\to\Real$ such that for all $c\in\mathcal C_X$, $f\circ c\in C^\infty(\Real,\Real)$ then $f\in\mathcal F_X$.
  \end{enumerate}
  A \emph{morphism} between Fr\"olicher spaces $(X,\mathcal C_X,\mathcal F_X)$ and $(Y,\mathcal C_Y,\mathcal F_Y)$ is a map $\phi\from X\to Y$ satisfying $f\circ\phi\circ c\in C^\infty(\Real,\Real)$ for all $f\in\mathcal F_Y$ and $c\in\mathcal C_X$.
\end{definition}
It is well-known that the category of Fr\"olicher spaces is cartesian closed.

We restrict this notion ever so slightly, assuming a vector space structure:
\begin{definition}
  A $\Real$-\emph{vector space Fr\"olicher space} (VFS) is a Fr\"olicher space $(X,\mathcal C_X,\mathcal F_X)$ such that $X$ is an $\mathcal R$-vector space and whenever $c,c'\in\mathcal C_X$ and $\alpha\in C^\infty(\Real,\Real)$ then $\alpha \, c+c'\in\mathcal C_X$ (defined pointwise).

  A \emph{morphism} between $\Real$-\emph{vector space Fr\"olicher spaces} is a morphism between Fr\"olicher spaces.
\end{definition}

\lo{Equivalent definition. A VFS is a Fr\"olicher space $(X,\mathcal C_X,\mathcal F_X)$ such that $X$ is a $\mathcal R$-vector space such that the scalar multiplication $\mathcal{R} \times X \to X$ and addition $X \times X \to X$ are smooth (meaning that they are Fr\"olicher space morphisms, where $\mathcal R$ is the so-called standard Fr\"olicher space).}

\lo{Remark. Another way to access vector space operations in the setting of Fr\"olicher spaces is via the (cartesian closed category of) convenient vector spaces, which may be viewed as Fr\"olicher spaces that are locally convex spaces with certain smooth curves and functionals.
However the approach via the subcategory of VFS seems fit for purpose and simpler.}

\begin{proposition}
  The $\Real$-\emph{vector space Fr\"olicher spaces} and their morphisms form a category which is cartesian closed.
\end{proposition}
\begin{proof}[Proof sketch]
  The proof for Fr\"olicher spaces carries over. In particular, for $(X,\mathcal C_X,\mathcal F_X)$ and $(Y,\mathcal C_Y,\mathcal F_Y)$,
  \begin{align*}
    X\Rightarrow Y&\defeq C^\infty(X,Y)\\
    \mathcal F&\defeq\{\phi\mapsto\psi(f_Y\circ\phi\circ c_X)\mid\psi\in C^\infty(\Real,\Real)'\land f_Y\in\mathcal F_Y\land c_X\in\mathcal C_X\}\\
    \mathcal C_{X\Rightarrow Y}&\defeq\{c\from\Real\to C^\infty(X,Y)\mid\forall f\in\mathcal F\ldotp f\circ c\in\mathcal C^\infty(\Real,\Real)\}\\
    \mathcal F_{X\Rightarrow Y}&\defeq\{f\from C^\infty(X,Y)\to\Real\mid\forall c\in\mathcal C_{X\Rightarrow Y}\ldotp f\circ c\in\mathcal C^\infty(\Real,\Real)\}
  \end{align*}
  where $E'$ is the set of bounded linear functionals $E\to\Real$, and
  $(\alpha\phi+\phi')(x)\defeq\alpha(x)\phi(x)+\phi'(x)$ for $\phi,\phi'\in C^\infty(X,Y)$, $\alpha\in C^\infty(\Real,\Real)$ and $x\in X$.
\end{proof}
\lo{Notation: I assume by $C^\infty(X,Y)$ you mean the hom-set in the category of VFS.} \dw{yes}

\lo{So the internal homset is the VFS object generated by the set of functionals $\mathcal F$.}

%\lo{Def.~of $\mathcal F$: prime in $C^\infty(\Real,\Real)'$ means its dual?}

Now, suppose
\begin{align*}
  \phi_1,\phi_2\from(X,\mathcal C_X,\mathcal F_X)&\to(Y,\mathcal C_Y,\mathcal F_Y)&
  \psi\from(X,\mathcal C_X,\mathcal F_X)&\to(\Real,\mathcal C_\Real,\mathcal F_\Real)
\end{align*}
are morphisms between VFS and $\eta>0$.

\changed[dw]{Writing $\sigma_\eta(x) := \sigma(\frac x\eta)= \frac{1}{1 + \exp(-\frac x\eta)}$}, we define
\begin{align*}
  \phi_1\brm\psi\eta\phi_2\from X&\to Y\\
  x&\mapsto(1-\sigma_\eta(\psi(x)))\cdot\phi_1(x)+\sigma_\eta(\psi(x))\cdot\phi_2(x)
\end{align*}
i.e.\ $\phi_1\brm\psi\eta\phi_2\defeq (1-\sigma_\eta\circ\psi)\phi_1+(\sigma_\eta\circ\psi)\phi_2$.
\begin{proposition}
  $\phi_1\brm\psi\eta\phi_2$ is a morphism $(X,\mathcal C_X,\mathcal F_X)\to(Y,\mathcal C_Y,\mathcal F_Y)$.
\end{proposition}
\begin{proof}
  It suffices to prove that for all $c\in\mathcal C_X$, $(\phi_1\brm\psi\eta\phi_2)\circ c\in\mathcal C_Y$. This is clear by definition and because $\sigma_\eta\circ\psi\circ c\in C^\infty(\Real,\Real)$ for $c\in\mathcal C_X$.
\end{proof}
Note that $\chi\circ(\phi_1\brm\psi\eta\phi_2)=(\chi\circ\phi_1)\brm\eta\psi(\chi\circ\phi_2)$.

%\lo{The notation $\phi_1 \oplus_\psi \phi_2$ is overloaded and confusing!}



\subsection{Value Semantics}
\begin{align*}
  \sem\PCFReal&\defeq\Real\\
  \sem\PCFRp&\defeq\Realp\\
  \sem{[\rbt_1,\ldots,\rbt_n]}&\defeq\sem{\rbt_1}\times\cdots\times\sem{\rbt_n}\\
  \sem{\sigma\trt\to\tau}&\defeq\sem\sigma\times\sem\trt\Rightarrow\sem\tau
\end{align*}
\dw{or list for semantics of $\trt$?}
\lo{What function space is $[\sem\sigma\times\sem\trt\to\sem\tau]$?}

\dw{Define $\sem{-}$ in QBS and $\sema-$ in Fr\"olicher}
Define $\sema{\Gamma\mid\trt\vdash M:\tau}:\sem\Gamma\times\sem\trt\to\sem\tau$:

\lo{Below: Corrected typo in if-branching; added rule for variable}
\begin{align*}
  \sema{\Gamma\mid[\PCFReal]\vdash\sample:\PCFReal}(\gamma,[s])&\defeq s\\
  \sema{\Gamma, x : \sigma \mid[]\vdash x : \sigma}((\gamma,v), [])&\defeq v\\
  \sema{\Gamma\mid[]\vdash\lambda y\ldotp M:\sigma\trt\to\tau}(\gamma,[])&\defeq\\
  &\hspace*{-3cm}(v,\tr)\in\sem\sigma\times\sem\trt\mapsto\sema{\Gamma,x:\sigma\mid\trt\vdash M:\tau}((\gamma,v),\tr)\\
  \sema{\Gamma\mid\trt\app\trt'\app\trt''\vdash M\,N:\tau}(\gamma,\tr\app\tr'\app\tr'')&\defeq\\
  &\hspace*{-3cm}\sema{\Gamma\mid\trt\vdash M:\sigma\trt''\to\tau}(\gamma,\tr)(\sema{\Gamma\mid\trt'\vdash N:\sigma}(\gamma,\tr'),\tr'')\\
  \sema{\Gamma\mid\trt\app\trt'\app\trt''\vdash\ifc LMN:\tau}(\gamma,\tr\app\tr'\app\tr'')&\defeq\\
  %&\hspace*{-3cm}\sigma_\eta(-\sema{\Gamma\mid\trt\vdash L:\PCFReal}(\gamma,\tr))\cdot\sema{\Gamma\mid\trt'\vdash M:\tau}(\gamma,\tau)\\
  %&\hspace*{-3cm}+\sigma_\eta(\sema{\Gamma\mid\trt\vdash L:\PCFReal}(\gamma,\tr))\cdot\sema{\Gamma\mid\trt''\vdash N:\tau}(\gamma,\tau)
  &\hspace*{-3cm}\sigma_\eta(-\sema{\Gamma\mid\trt\vdash L:\PCFReal}(\gamma,\tr))\cdot\sema{\Gamma\mid\trt'\vdash M:\tau}(\gamma,\tr')\\
  &\hspace*{-3cm}+\sigma_\eta(\sema{\Gamma\mid\trt\vdash L:\PCFReal}(\gamma,\tr))\cdot\sema{\Gamma\mid\trt''\vdash N:\tau}(\gamma,\tr'')
\end{align*}

\dw{branches with higher-order: vector space}
\dw{transformed sample}

\begin{lemma}[Substitution]
  $\sema {M[V/x]}(\gamma,\tr)=\sema M (\gamma[x\mapsto\sema V(\gamma,[])],\tr)$.
\end{lemma}
Note that the restrictions to values is essential. E.g. for $(x+x)[\sample/x]$ a similar property does not hold. On the other hand, $(f\,0+f\,0)[(\lambda x\ldotp\sample)/y]$ is not problematic.

\begin{proposition}[Soundness]
  If $M\Downarrow_\tr V$ then $\sema M(\gamma,\tr)=\sema V(\gamma,[])$.
\end{proposition}

\dw{differentiable, ensure other properties}

%\input{value-semantics-alternative}

